Revitalize Region Feature for Democratizing Video-Language Pre-training of Retrieval

Recent dominant methods for video-language pre-training (VLP) learn transferable representations from the raw pixels in an end-to-end manner to achieve advanced performance on downstream video-language retrieval. Despite the impressive results, VLP research becomes extremely expensive with the need for massive data and a long training time, preventing further explorations. In this work, we revitalize region features of sparsely sampled video clips to significantly reduce both spatial and temporal visual redundancy towards democratizing VLP research at the same time achieving state-of-the-art results. Specifically, to fully explore the potential of region features, we introduce a novel bidirectional region-word alignment regularization that properly optimizes the fine-grained relations between regions and certain words in sentences, eliminating the domain/modality disconnections between pre-extracted region features and text. Extensive results of downstream video-language retrieval tasks on four datasets demonstrate the superiority of our method on both effectiveness and efficiency, \textit{e.g.}, our method achieves competing results with 80\% fewer data and 85\% less pre-training time compared to the most efficient VLP method so far \cite{lei2021less}. The code will be available at \url{https://github.com/showlab/DemoVLP}.

==> arxiv_tables/comp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
% \vspace{-4mm}
\begin{tabular}{c|c|c|c|lll}
\hline
                                     &                                      &                                &                                  & \multicolumn{3}{c}{Text$\rightarrow$Video} \\
\multirow{-2}{*}{Refine Attention}   & \multirow{-2}{*}{Select Token}       & \multirow{-2}{*}{Track Object} & \multirow{-2}{*}{Temporal Model} & R@1    & R@5   & R@10 \\ \hline
-                                    & -                                    & -                              & -                                &    34.5    &  58.3     &  70.2    \\
\rowcolor{LightCyan} 
$\checkmark$                         & -                                    & -                              & -                                & \textbf{36.0}   & \textbf{61.0}  & \textbf{71.8}     \\
-            & $\checkmark$ & -                              & -                                &    32.8    &  55.5     &  69.2        \\
$\checkmark$ & -                                    & $\checkmark$                   & -                                & 33.6   & 59.2  & 69.7    \\
$\checkmark$ & -                                    & -                              & $\checkmark$                     & 35.9   & 60.8  & 71.8     \\ \hline
\end{tabular}
\vspace{2mm}
\caption{Ablation study of different model explorations. The first row denotes a baseline and the colored row denotes our method.}
\label{tab:ablation}
% \vspace{-8mm}
\end{table}

==> arxiv_tables/data-scale-gene.tex <==
\begin{figure}
% \vspace{-6mm}
     \centering
     \begin{minipage}[b]{0.5\columnwidth}
         \centering
         \begin{tabular}{c|lll}
\hline
\multirow{2}{*}{Data} & \multicolumn{3}{c}{Text$\rightarrow$Video} \\
                      & R@1      & R@5      & R@10     \\ \hline
WebVid+CC3M           & 36.0     & 61.0     & 71.8     \\
CC3M+CC7M             & 38.7     & 63.8     & \textbf{73.9}     \\
WebVid+CC3M+CC7M      & \textbf{39.6}     & \textbf{64.8}     & 73.8     \\ \hline
\end{tabular}
        \vspace{6mm}
         \tabcaption{Generalize to more data.}
         \label{tab:data-gene}
     \end{minipage}
     \hfill
     \begin{minipage}[b]{0.45\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/data-scale-fig.pdf}
         \caption{Effect of different data scales.}
         \label{fig:data-scale}
     \end{minipage}
        % \caption{(a) Effectiveness of region-word alignment. (b) Impact of frame number.}
        \label{fig:data-scale-gene}
        % \vspace{-4mm}
\end{figure}

==> arxiv_tables/infer-time-all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
% \vspace{-8mm}
\begin{tabular}{l|cc|cc}
\hline
\multirow{2}{*}{Components} & \multicolumn{2}{c|}{12000 Samples}                                   & \multicolumn{2}{c}{1000 Samples}                                     \\ \cline{2-5} 
                            & \multicolumn{1}{c|}{Text$\rightarrow$Video} & Video$\rightarrow$Text & \multicolumn{1}{c|}{Text$\rightarrow$Video} & Video$\rightarrow$Text \\ \hline
Language Encoder            & \multicolumn{1}{c|}{5.6ms}                  & -                      & \multicolumn{1}{c|}{4.8ms}                  & -                      \\
Video Encoder               & \multicolumn{1}{c|}{-}                      & 17.6ms                 & \multicolumn{1}{c|}{-}                      & 16.4ms                 \\
Detector                    & \multicolumn{1}{c|}{-}                      & 103.2ms                & \multicolumn{1}{c|}{-}                      & 103.2ms                \\ \hline
Rank                        & \multicolumn{1}{c|}{372.2ms}                & 345.8ms                & \multicolumn{1}{c|}{31.8ms}                 & 30.0ms                 \\ \hline
\end{tabular}
\vspace{3mm}
\caption{Inference time of each model component. Because the length of sentence and size of video frames are different in WebVid and LSMDC, inference time on language and video encoders is different.}
\vspace{-8mm}
\label{tab:infer-time-all}
\end{table}

==> arxiv_tables/num-frame-object.tex <==
\begin{figure}
% \vspace{-6mm}
     \centering
     \begin{minipage}[b]{0.48\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/num-object.pdf}
         \caption{Different number of objects.}
         \label{fig:num-obj}
     \end{minipage}
     \hfill
     \begin{minipage}[b]{0.48\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/num-frame.pdf}
         \caption{Different number of frames.}
         \label{fig:num-frame}
     \end{minipage}
        % \caption{(a) Effectiveness of region-word alignment. (b) Impact of frame number.}
        \label{fig:num-obj-frame}
        % \vspace{-4mm}
\end{figure}

==> arxiv_tables/pretrain-time.tex <==
\begin{figure}
% \vspace{-4mm}
     \centering
     \begin{minipage}[b]{0.48\columnwidth}
         \centering
         \begin{tabular}{l|c|c|c}
            \hline
            \textbf{Method} & \textbf{Data} & \textbf{GPU Hrs} & \textbf{R@1} \\ \hline
            Frozen~\cite{Bain_2021_ICCV}          & 5.8M                & 4800      & 31.0         \\
            UniVL~\cite{luo2020univl}           & 132M                & 2496           & 21.2   \\       
            HERO~\cite{li2020hero}            & 7.6M                & 8064             & 20.5  \\
            VIOLET~\cite{fu2021violet}          & 185.8M              & 2240        &   34.5    \\
            ClipBERT~\cite{lei2021less}        & 5.6M                & 768              & 22.0  \\ \hline
            Ours (4F/1.0) & 5.8M                & 1600      & 36.3         \\
            Ours (1F/1.0) & 5.8M                & 800      & 36.0          \\
            Ours (1F/0.5)  & 2.9M                & 416       & 36.4        \\
            Ours (1F/0.2)  & 1.2M                & 104      & 34.6          \\ \hline
        \end{tabular}%
         \tabcaption{Comparing the pre-training efficiency with existing video-language pre-training methods. 4F means that 4 frames per video are sampled for pre-training. 0.2 means that only 20\% pre-training data are used.}
         \label{tab:pretrain-time}
     \end{minipage}
     \hfill
     \begin{minipage}[b]{0.48\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/train-time.pdf}
         \vspace{0.5mm}
         \caption{Comparing the running time of a training loop with existing video-language pre-training methods. Batchsize is set to 16 and mixed precision is disabled for all methods.}
         \label{fig:train-time}
     \end{minipage}
        % \caption{(a) Effectiveness of region-word alignment. (b) Impact of frame number.}
        \label{fig:pretrain-train-time}
        % \vspace{-8mm}
\end{figure}

==> arxiv_tables/retrieval.tex <==
\begin{table}[t]
% \vspace{-5mm}
    \begin{subtable}[h]{0.44\textwidth}
        \centering
        \begin{tabular}{llll}
            \hline
            \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{Text$\rightarrow$Video}}                       \\
            \multicolumn{1}{l|}{}                                 & \textbf{R@1}  & \textbf{R@5}  & \textbf{R@10}  \\ \hline
            \multicolumn{1}{l|}{JSFusion~\cite{yu2018joint}}                         & 9.1           & 21.2          & 34.1                    \\
            \multicolumn{1}{l|}{MEE~\cite{miech2018learning}}                              & 9.3           & 25.1          & 33.4                    \\
            \multicolumn{1}{l|}{CE~\cite{liu2019use}}                               & 11.2          & 26.9          & 34.8                   \\
            \multicolumn{1}{l|}{MMT~\cite{gabeur2020multi}}                              & 12.9          & 29.2          & 38.8                    \\
            \multicolumn{1}{l|}{AVLNet~\cite{rouditchenko2021cascaded}}                           & 17.0          & 38.0          & 48.6                    \\
            \multicolumn{1}{l|}{Dig~\cite{wang2021dig}}                              & 15.8          & 34.1          & 43.6                    \\
            \multicolumn{1}{l|}{Frozen~\cite{Bain_2021_ICCV}}                           & 15.0          & 34.1          & 39.8                    \\
            \multicolumn{1}{l|}{VTMCE~\cite{ali2022video}}                           & 14.9          & 33.2          & -                    \\
            \multicolumn{1}{l|}{MDMMT~\cite{dzabraev2021mdmmt}}                           & 18.8          & 38.5          & 47.9                    \\
            \multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{25.2} & \textbf{45.5} & \textbf{54.5}   \\ \hline
            \multicolumn{4}{l}{Zero-shot}                                                                                         \\ \hline
            \multicolumn{1}{l|}{Ours}                             & 14.3          & 25.8          & 32                     \\ \hline
            \end{tabular}%
       \caption{LSMDC retrieval}
       \label{tab:lsmdc_retrieval}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.44\textwidth}
        \centering
        \begin{tabular}{llll}
            \hline
            \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{Text$\rightarrow$Video}}                       \\
            \multicolumn{1}{l|}{}                                 & \textbf{R@1}  & \textbf{R@5}  & \textbf{R@10}  \\ \hline
            \multicolumn{1}{l|}{MMT~\cite{gabeur2020multi}}                              & 26.6          & 57.1          & 69.6                     \\
            \multicolumn{1}{l|}{ActBERT~\cite{zhu2020actbert}}                          & 16.3          & 42.8          & 56.9                    \\
            \multicolumn{1}{l|}{SupportSet~\cite{patrick2021supportset}}                       & 30.1          & 58.5          & 69.3                     \\
            \multicolumn{1}{l|}{AVLNet~\cite{rouditchenko2021cascaded}}                           & 27.1          & 55.6          & 66.6                     \\
            \multicolumn{1}{l|}{TACo~\cite{yang2021taco}}                             & 29.6          & 59.7          & \textbf{72.7}                    \\
            \multicolumn{1}{l|}{ClipBERT~\cite{lei2021less}}                         & 22.0          & 46.8          & 59.9                    \\
            \multicolumn{1}{l|}{Frozen~\cite{Bain_2021_ICCV}}                           & 31.0          & 59.5 & 70.5                     \\
            \multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{36.0} & \textbf{61.0}          & 71.8   \\ \hline
            \multicolumn{4}{l}{Zero-shot}                                                                                         \\ \hline
            \multicolumn{1}{l|}{SupportSet~\cite{patrick2021supportset}}                       & 12.7          & 27.5          & 36.2                  \\
            \multicolumn{1}{l|}{Frozen~\cite{Bain_2021_ICCV}}                           & 18.7          & 39.5          & 51.6                    \\
            \multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{24.0} & \textbf{44.0} & \textbf{52.6}   \\ \hline
        \end{tabular}%
        \caption{MSRVTT retrieval}
        \label{tab:msrvtt_retrieval}
     \end{subtable}
     \hfill
     \begin{subtable}[h]{0.44\textwidth}
        \centering
        \begin{tabular}{llll}
            \hline
            \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{Text$\rightarrow$Video}}                       \\
            \multicolumn{1}{l|}{}                                 & \textbf{R@1}  & \textbf{R@5}  & \textbf{R@10}  \\ \hline
            \multicolumn{1}{l|}{S2VT~\cite{venugopalan2014translating}}                             & 11.9          & 33.6          & -                       \\
            \multicolumn{1}{l|}{FSE~\cite{zhang2018cross}}                              & 13.9          & 36.0          & -                      \\
            \multicolumn{1}{l|}{CE~\cite{liu2019use}}                              & 16.1          & 41.1          & 54.4                      \\
            \multicolumn{1}{l|}{ClipBERT~\cite{lei2021less}}                         & 20.4          & 44.5          & 56.7                     \\
            \multicolumn{1}{l|}{Frozen~\cite{Bain_2021_ICCV}}                           & 31.0          & 59.8          & 72.4                     \\ 
            \multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{41.4} & \textbf{67.6} & \textbf{77.6}   \\ \hline
            \multicolumn{4}{l}{Zero-shot}                                                                                         \\ \hline
            \multicolumn{1}{l|}{Frozen~\cite{Bain_2021_ICCV}}                           & 21.1          & 46.0          & 56.2                     \\
            \multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{29.6} & \textbf{53.0} & \textbf{65.1}  \\ \hline
        \end{tabular}%
        \caption{DiDeMo retrieval}
        \label{tab:didemo_retrieval}
     \end{subtable}
     \hfill
     \begin{subtable}[h]{0.44\textwidth}
        \centering
        \begin{tabular}{llll}
            \hline
            \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{Text$\rightarrow$Video}}                       \\
            \multicolumn{1}{l|}{}                                 & \textbf{R@1}  & \textbf{R@5}  & \textbf{R@10}  \\ \hline
            \multicolumn{1}{l|}{VSE~\cite{kiros2014unifying}}                              & 12.3          & 30.1          & 42.3                  \\
            \multicolumn{1}{l|}{VSE++~\cite{faghri2017vse++}}                            & 15.4          & 39.6          & 53.0                    \\
            \multicolumn{1}{l|}{MCues~\cite{mithun2018learning}}                            & 20.3          & 47.8          & 61.1                    \\
            \multicolumn{1}{l|}{CE~\cite{liu2019use}}                               & 19.8          & 49.0          & 63.8                    \\
            \multicolumn{1}{l|}{SupportSet~\cite{patrick2021supportset}}                       & 28.4          & 60.0          & 72.9                     \\
            \multicolumn{1}{l|}{Frozen~\cite{Bain_2021_ICCV}}                           & 33.7          & 64.7          & 76.3                    \\
            \multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{50.9} & \textbf{78.9} & \textbf{87.0}   \\ \hline
            \multicolumn{4}{l}{Zero-shot}                                                                                         \\ \hline
            \multicolumn{1}{l|}{Ours}                    & 41.6 & 69.8 & 80.5    \\ \hline
        \end{tabular}%
        \caption{MSVD retrieval}
        \label{tab:msvd_retrieval}
     \end{subtable}
     \caption{Comparisons with state-of-the-art results on video-language retrieval.}
     \label{tab:video_retrieval}
    %  \vspace{-9mm}
\end{table}

==> arxiv_tables/rwa-new.tex <==
\begin{table}[h]
% \vspace{-6mm}
    \begin{subtable}[h]{0.5\textwidth}
        \centering
        \begin{tabular}{l|lll}
\hline
\multirow{2}{*}{Method} & \multicolumn{3}{c}{Text$\rightarrow$Video} \\
                        & R@1      & R@5      & R@10     \\ \hline
Base                    & 22.5     & 48.1     & 59.5     \\ \hline
TACo~\cite{yang2021taco}               & 29.6     & 59.7     & \textbf{72.7}        \\
Base+TACo               & 29.8     & 60.1     & 70.7        \\ 
Base+FILIP              & 27.8        & 55.0        & 65.1       \\ \hline
Ours(Base+RWA)          & \textbf{36.0}     & \textbf{61.0}     & 71.8     \\ \hline
\end{tabular}
       \caption{Comparison with other visual-language alignment methods on MSRVTT retrieval.}
       \label{tab:rwa-effect}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.5\textwidth}
        \centering
        \begin{tabular}{llll}
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{Method}} & \multicolumn{3}{c}{Text$\rightarrow$Video} \\
\multicolumn{1}{l|}{}                        & R@1          & R@5          & R@10         \\ \hline
\multicolumn{1}{l|}{Frozen}                  & 31.0         & 59.5         & 70.5         \\ 
\multicolumn{1}{l|}{Frozen+RWA}              & 35.1         & 60.7         & 70.9         \\ \hline
\multicolumn{4}{l}{Zero-shot}                                                             \\ \hline
\multicolumn{1}{l|}{Frozen}                  & 18.7         & 39.5         & 51.6         \\ 
\multicolumn{1}{l|}{Frozen+RWA}              & 21.7         & 42.2         & 52.2         \\ \hline
\end{tabular}
        \caption{Results on MSRVTT retrieval when cooperating with Frozen.}
        \label{tab:rwa-gene}
     \end{subtable}
     \caption{Effectiveness and generalization ability of our region-word alignment.}
     \label{tab:rwa-new}
    %  \vspace{-10mm}
\end{table}

==> arxiv_tables/video-qa.tex <==
\begin{table}[t]
% \vspace{-4mm}
    \begin{subtable}[h]{0.5\textwidth}
        \centering
        \begin{tabular}{l|c}
            \hline
            \textbf{Method} & \multicolumn{1}{l}{\textbf{MSRVTT}} \\ \hline
            JSFusion~\cite{yu2018joint}        & 83.4                                \\
            ActBERT~\cite{zhu2020actbert}         & 85.7                                \\
            ClipBERT~\cite{lei2021less}        & 88.2                                \\
            VideoCLIP~\cite{xu2021videoclip}       & 92.1                                \\
            MERLOT~\cite{zellersluhessel2021merlot}          & 90.9                                \\
            VIOLET~\cite{fu2021violet}          & 91.9                                \\ \hline
            \textbf{Ours}   & \textbf{92.4}                       \\ \hline
            \end{tabular}%
       \caption{MSRVTT Multiple Choice}
       \label{tab:msrvtt_mc}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.5\textwidth}
        \centering
        \begin{tabular}{l|c|c}
            \hline
            \textbf{Method} & \multicolumn{1}{l|}{\textbf{MSRVTT}} & \multicolumn{1}{l}{\textbf{MSVD}} \\ \hline
            Co-Mem~\cite{gao2018motion}            & 32.0                                & 31.7                              \\
            HMEMA~\cite{fan2019heterogeneous}            & 33.0                                & 33.7                              \\
            SSML~\cite{Amrani_Ben-Ari_Rotman_Bronstein_2021}            & 35.0                                & 35.1                              \\
            HCRN~\cite{le2020hierarchical}            & 35.6                                & 36.1                              \\
            DualVGR~\cite{wang2021dualvgr}         & 35.5                                & 39.0                              \\
            ClipBERT~\cite{lei2021less}        & 37.4                                & -                                 \\
            % JustAsk~\cite{Yang_2021_ICCV}         & 43.1                                & 46.3                              \\
            % VIOLET~\cite{fu2021violet}          & 43.9                                & 47.9                              \\ \hline
            \hline
            \textbf{Ours}            & \textbf{38.3}                                & \textbf{39.5}                              \\ \hline
            \end{tabular}%
        \caption{MSRVTT QA and MSVD QA}
        \label{tab:msrvtt_msvd_qa}
     \end{subtable}
     \caption{Comparisons with state-of-the-art results on video question answering.}
     \label{tab:video_qa}
    %  \vspace{-6mm}
\end{table}

==> arxiv_tables/vis.tex <==
\begin{figure}[t]
% \vspace{-27mm}
     \centering
     \begin{subfigure}[b]{0.48\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/region-word-vis_cropped.pdf}
         \caption{Attended regions with respect to the most relevant word in the corresponding sentence.}
         \label{fig:region-word-vis}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/video-caption-vis_cropped.pdf}
         \vspace{-30mm}
         \caption{Attention heatmap of video frames and corresponding sentence. Relevant regions are highlighted.}
         \label{fig:video-caption-vis}
     \end{subfigure}
        \caption{Visualization of the alignment between video and language.}
        \label{fig:vis}
        % \vspace{-6mm}
\end{figure}

==> figs/comp-infer.tex <==
\begin{figure}
     \centering
     \begin{minipage}[b]{0.48\columnwidth}
         \centering
         \begin{tabular}{c|c|c|c|lll}
\hline
Select & Refine & Object & Temp & \multicolumn{3}{c}{Text Video} \\
Token  & attn   & Track  & Attn & R@1      & R@5      & R@10     \\ \hline
-      & -      & -      & -    & 36.0     & 61.0     & 71.8     \\
$\checkmark$      & -      & -      & -    &          &          &          \\
-      & $\checkmark$      & -      & -    &          &          &          \\
-      & -      & $\checkmark$      & -    & 33.6     & 59.2     & 69.7     \\
-      & -      & -      & $\checkmark$    & 35.9     & 60.8     & 71.8     \\ \hline
\end{tabular}
         \tabcaption{Ablation study of each model design.}
         \label{tab:comp}
     \end{minipage}
     \hfill
     \begin{minipage}[b]{0.48\columnwidth}
         \centering
\begin{tabular}{l|c|c}
\hline
Components & Text Video             & \multicolumn{1}{c|}{Video Text} \\ \hline
Language   & \multirow{2}{*}{5.6ms} & \multirow{2}{*}{-}              \\
Encoder    &                        &                                 \\ \hline
Video      & \multirow{2}{*}{-}     & \multirow{2}{*}{17.6ms}         \\
Encoder    &                        &                                 \\ \hline
Detect     & -                      & 103.2ms                         \\ \hline
Rank       & 372.2ms                & 345.8ms                         \\ \hline
\end{tabular}
         \tabcaption{Inference time of model components.}
         \label{tab:infer-time}
     \end{minipage}
        % \caption{(a) Effectiveness of region-word alignment. (b) Impact of frame number.}
        \label{fig:comp-infer-time}
\end{figure}

==> figs/data-scale-gene.tex <==
\begin{figure}
\vspace{-6mm}
     \centering
     \begin{minipage}[b]{0.5\columnwidth}
         \centering
         \begin{tabular}{c|lll}
\hline
\multirow{2}{*}{Data} & \multicolumn{3}{c}{Text$\rightarrow$Video} \\
                      & R@1      & R@5      & R@10     \\ \hline
WebVid+CC3M           & 36.0     & 61.0     & 71.8     \\
CC3M+CC7M             & 38.7     & 63.8     & \textbf{73.9}     \\
WebVid+CC3M+CC7M      & \textbf{39.6}     & \textbf{64.8}     & 73.8     \\ \hline
\end{tabular}
        \vspace{6mm}
         \tabcaption{Generalize to more data.}
         \label{tab:data-gene}
     \end{minipage}
     \hfill
     \begin{minipage}[b]{0.45\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/data-scale-fig.pdf}
         \caption{Effect of different data scales.}
         \label{fig:data-scale}
     \end{minipage}
        % \caption{(a) Effectiveness of region-word alignment. (b) Impact of frame number.}
        \label{fig:data-scale-gene}
        \vspace{-4mm}
\end{figure}

==> figs/data-scale.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.49\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/local-data-scale.pdf}
         \caption{Finetuning and zero-shot results with region-word alignment.}
         \label{fig:local-data-scale}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/global-data-scale.pdf}
         \caption{Finetuning and zero-shot results without region-word alignment.}
         \label{fig:global-data-scale}
     \end{subfigure}
        \caption{Effect of different data scales.}
        \label{fig:data_scale}
\end{figure}

==> figs/num-frame-obj.tex <==
\begin{figure}
\vspace{-6mm}
     \centering
     \begin{minipage}[b]{0.48\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/num-object.pdf}
         \caption{Different number of objects.}
         \label{fig:num-obj}
     \end{minipage}
     \hfill
     \begin{minipage}[b]{0.48\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/num-frame.pdf}
         \caption{Different number of frames.}
         \label{fig:num-frame}
     \end{minipage}
        % \caption{(a) Effectiveness of region-word alignment. (b) Impact of frame number.}
        \label{fig:num-obj-frame}
        \vspace{-4mm}
\end{figure}

==> figs/rwa+sampling.tex <==
\begin{figure}
     \centering
     \begin{minipage}[b]{0.45\columnwidth}
         \centering
         \begin{tabular}{lllll}
            \hline
            \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{4}{c}{\textbf{Text Video}}                       \\
            \multicolumn{1}{l|}{}                                 & \textbf{R@1}  & \textbf{R@5}  & \textbf{R@10} & \textbf{MedR} \\ \hline
            \multicolumn{1}{l|}{Frozen+RWA}                       & 35.1          & 60.7          & 70.9          & 3.0           \\
            \multicolumn{1}{l|}{Frozen}                           & 31.0          & 59.5 & 70.5          & 3.0           \\ \hline
            \multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{36.0} & \textbf{61.0}          & \textbf{71.8} & \textbf{3.0}  \\
            \multicolumn{1}{l|}{Ours w/o RWA}                     & 22.5          & 48.1          & 59.5          & 6.0           \\ \hline
            Zero-shot                                             &               &               &               &               \\ \hline
            \multicolumn{1}{l|}{Frozen+RWA}                       & 20.1          & 37.5          & 49.3          & 11.0          \\
            \multicolumn{1}{l|}{Frozen}                           & 18.7          & 39.5          & 51.6          & 10.0          \\ \hline
            \multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{24.0} & \textbf{44.0} & \textbf{52.6} & \textbf{8.0}  \\
            \multicolumn{1}{l|}{Ours w/o RWA}                     & 16.1          & 34.9          & 44.2          & 16.0          \\ \hline
        \end{tabular}%
         \tabcaption{Effect of region-word alignment on our method and Frozen.}
         \label{tab:rwa}
     \end{minipage}
     \hfill
     \begin{minipage}[b]{0.51\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/num-frame.pdf}
         \vspace{-8mm}
         \caption{Effect of different number of frames.}
         \label{fig:frame-number}
     \end{minipage}
        % \caption{(a) Effectiveness of region-word alignment. (b) Impact of frame number.}
        \label{fig:rwa+frame-number}
\end{figure}

==> rebuttal_tables/ToAC.tex <==
\noindent Dear AC,

Thanks for handling our submission.

% limited contribution; democratize VLP -> encourage more people do research in this field -> produce more interesting works.
% for the technical novelty; first prove region features can perform well on video-text pretrain; recent dominant opinion is that e2e models are more efficient and effective than offline-feature-based models;
We want to emphasize that our model is the first to introduce region features to democratize video-text pretrain.
Recent end-to-end methods require massive data and long pretrain time, which prevent most researchers from this field.
Based on our efficient model, more researchers can be involved to explore interesting findings in this field.
From the perspective of technical contribution, we explored several potential directions to make offline-feature-based models efficient and powerful (e.g., sparse sampling, video-text alignment, temporal modeling), which can inspire not only offline-feature-based works, but also end-to-end works in the future. 

% misunderstanding of temporal modeling
Beyond that, we want to point out that reviewers have some misunderstandings of our work.
All reviewers argue that our model cannot capture temporal information in videos.
However, we have already described how our model captures dynamic content in videos.
Ablation study of temporal modeling is also given.

% misunderstanding of other points
% 1. refinement; no evidence of off-the-shelf features were unsuccessful due to sub-optimal regularization; 
% 2. results with more frames
% 3. time analysis on downstream tasks.
R1 argues that the proposed refinement lacks ablation study.
In fact, we have also given it in Table 7.
R1 also argues that we didn't give evidence of off-the-shelf features not being successful.
However, in Table 4 and Section 4.4, we have given such evidence from two perspectives.
% However, in Table 4, we have shown that previous offline-feature-based methods are surpassed by end-to-end methods.
% Meanwhile, in Section 4.4, we analyzed that off-the-shelf features can only get poor performance without RWA.

R2 has a misunderstanding of the results in Fig.6, and argues that our method doesn't capture actions based on such misunderstanding.
In our response, we give a detailed explanation of this misunderstanding, and prove that our model indeed captures actions in videos.

R3 argue that time analysis on downstream tasks is lacked.
However, the analysis is given in Section 3.4.

We acknowledge that the current version of our manuscript has some flaws, e.g., unclear descriptions of temporal modeling lead to misunderstanding by reviewers. We will make it clear. We sincerely hope you could rethink our paper, as our contribution to democratizing VLP research is indeed a knowledge advancement for the community.

\noindent Best,

\noindent Authors

==> rebuttal_tables/action.tex <==
\captionsetup{font={small}}

\begin{wraptable}{c}{3.5cm}
\scriptsize
\vspace{-5mm}
 \setlength{\abovecaptionskip}{0cm}
    \centering
    %\footnotesize
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|lll|l}
    %\toprule
    \hline
    Method & S1 & S2 & S3 & Mean \\
    %\midrule
    \hline
    ClipBERT & 18.8 & 19.4 & 19.6 & 19.3 \\
    Ours & 20.9 & 19.5 & 19.5 & 20.0\\
    %\bottomrule
    \hline
    \end{tabular}
    }
    \caption{Results of zero-shot action recognition.}
    %\caption{Computational analysis of retrieval in different scales of datasets. The time statistics is the average of 1,000 runs.}
    % , we report the average time of per video-text pair.}
    \vspace{-6mm}%%%%%%%%%%%%%%%%%%%%缩减竖直距离%%%%%%%%%%%%%%%%%%%%%%
    \label{tab:action}
\end{wraptable}

==> rebuttal_tables/num_frames_finetune.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\captionsetup{font={small}}
\setlength{\columnsep}{1em}%
\begin{wraptable}{c}{3cm}
\vspace{-5mm}
\scriptsize
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|c}
\hline
Num & Text$\rightarrow$Video \\ \hline
1   & 26.4/47.2/56.3         \\
2   & 29.9/53.7/64.3         \\
4   & 34.4/57.8/69.1         \\
6   & 35.1/59.3/69.9         \\
8   & 36.0/61.0/71.8         \\ \hline
Num & Video$\rightarrow$Text \\ \hline
8   & 32.7/58.4/68.4         \\ \hline
\end{tabular}%
}
\vspace{-3mm}
\caption{R@1/ R@5/ R@10 results of different number of frames during finetune.}
\vspace{-5mm}
\label{tab:num_frames_finetune}
\end{wraptable}

==> rebuttal_tables/temporal.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\captionsetup{font={small}}
\setlength{\columnsep}{1em}%
\begin{wraptable}{c}{3cm}
\vspace{-4mm}
\scriptsize
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|c}
\hline
Method & Text$\rightarrow$Video \\ \hline
w/o TPE     & 35.5/60.1/70.2         \\
TA     & 35.9/60.8/71.8         \\
TPE    & 36.0/61.0/71.8         \\ \hline
\end{tabular}%
}
\vspace{-3mm}
\caption{R@1/ R@5/ R@10 results of different temporal modeling. TA is time attention.}
\vspace{-5mm}
\label{tab:temporal}
\end{wraptable}

==> sections/1-Intro-revise-yxge.tex <==
\section{Introduction}
% 1. vlp发展，用于很多vl tasks；e2e方法dominate，但pretrain需要大量数据，并十分耗时，许多researcher难以展开vlp研究；democratization包括两方面：1. efficient 2. generality
% 2. efficient: clean data可以达到小规模数据，效果更佳->同理，raw image有噪声信息，region feature有更多有效信息->clipbert指出modality 和task的disconnection导致offline feature效果不佳->我们认为效果不佳的原因是用的方法不对，我们的loss如何解决了这两个disconnection
% 3. generality: real democratize需要我们方法上的strategy同样可以generalize到e2e的方法上；empirical study证明我们的loss可以适用于e2e patch方法和e2e region方法；
% contribution: 1 democratize vlp model: efficient and generalization; 2. new loss to better align video-text; 3. experimental results

% 1. video-language pre有更多有效信息；-training； VLP发展，可以用于很多downstream tasks；e2e方法dominated，但是十分耗时，许多researcher难以开展vlp研究
% Video-language tasks, such as text-video retrieval~\cite{lee2018stacked,liu2019focus}, video question answering~\cite{anderson2018bottom} and video captioning~\cite{anderson2018bottom,sharma2018conceptual}, require joint learning of video and language representations. 
% Recently, the pre-training-and-then-finetuning scheme~\cite{Bain_2021_ICCV,lei2021less,li2020hero,miech2020end} has become the most popular practice to cope with these tasks.
% % The typical paradigm of video-language pre-training (VLP) is to learn to fuse video-language representations based on pre-extracted video and language features using Transformers~\cite{vaswani2017attention}.
% % extract video and language features and then fuse them to learn a join video-language representations. 
% % Generally, the textual encoder and fusion module is based on Transformer~\cite{vaswani2017attention}.
% % As for the video encoder, most VLP methods~\cite{li2020hero,yu2018joint,gabeur2020multi,zhu2020actbert} utilize pre-trained action recognition models~\cite{feichtenhofer2019slowfast,hara2018can} to extract video features. 
% And the end-to-end methods~\cite{Bain_2021_ICCV,lei2021less,zellersluhessel2021merlot} have dominated this line of research by learning video-language representation from raw pixels and texts.
% % 2. faces problems: 1) require massive data->cost a lot of pre-training time; 2) lack a strong fine-grained alignment between video-language；现有的方法需要大量的数据和很长的pretrain时间，不论是offline还是e2e的方法；同时，由于Transformer backbone和处理video已经占用了大量的计算资源和显存，缺乏对于video-language的fine-grained alignment设计。
% Despite their significant progress in downstream performance, such methods are quite data-hungry due to a large number of model parameters and uncurated raw inputs.
% The pre-training stage turns out to be inefficient and expensive with massive pre-training data and long pre-training time, which causes many researcher hard to pursue research in VLP.



Video-language pre-training (VLP)~\cite{Bain_2021_ICCV,lei2021less,li2020hero,miech2020end} that jointly learns video and language representations in a self-supervised manner has become the most popular practice to cope with video-language tasks, such as text-to-video retrieval~\cite{lee2018stacked,liu2019focus} and video question answering~\cite{anderson2018bottom}.
% and video captioning~\cite{anderson2018bottom,sharma2018conceptual}.
% The typical paradigm of existing VLP approaches is to extract video and language features and then fuse them to learn a join video-language representations. 
% Generally, the textual encoder and fusion module is based on Transformer~\cite{vaswani2017attention}.
% As for the video encoder, most VLP methods~\cite{li2020hero,yu2018joint,gabeur2020multi,zhu2020actbert} utilize pre-trained action recognition models~\cite{feichtenhofer2019slowfast,hara2018can} to extract video features. 
% Recent methods~\cite{Bain_2021_ICCV,lei2021less,zellersluhessel2021merlot} attempt to develop end-to-end VLP models that learn video representation from raw pixels.
Recently, end-to-end methods~\cite{Bain_2021_ICCV,lei2021less,zellersluhessel2021merlot} that learn video representations from raw pixels have dominated due to their strong performance on downstream tasks.
% However, they still suffer from the requirement of massive pre-training data and long pre-training time, which causes many researcher hard to pursue research in VLP.
Despite significant progress, these methods are quite data-hungry due to a large number of model parameters and uncurated raw inputs.
The pre-training stage turns out to be inefficient and expensive with massive pre-training data and long pre-training time, making it difficult for researchers to pursue research in VLP.
\input{figs/intro}

% 2. existing methods tries to democratize VLP: 1. high-quality data; 2. temporal sparse sampling. ->core idea: remove noisy data -> region, spatial sparse sampling -> revitalize region features in previous image-text tasks -> accelerate pre-training
Previous work \cite{lei2021less} attempts to lower the barrier for VLP via removing visual redundancy. 
They point out that video clips with sparsely sampled frames are sufficient enough to capture key semantics for pre-training, since adjacent frames often contain similar scenes.
The effort enables more efficient VLP with competitive downstream performances. 
Besides the temporal visual redundancy, we argue that, in contrast to the text with highly abstract semantics, each frame of the video clips also has heavy spatial redundancy.
% , which prevents pre-training from further improving efficiency.

% from two perspectives: 
% % have explored efficient VLP models from two perspectives: 
% \textit{i) Data reduction:} datasets with high-quality captions can greatly alleviate the need for pre-training data.
% For example, Frozen~\cite{Bain_2021_ICCV} proposed a cleaner WebVid2.5M, which is 20x smaller than the widely-used dataset HowTo100M~\cite{miech2019howto100m}, to perform competitive VLP in a more efficient manner.
% % replace the most common used dataset, HowTo100M~\cite{miech2019howto100m}.
% % Compared with the large-scale noisy datasets, a clean dataset reduces the needed amount of pre-training data to less than 10 million.
% % The hypothesis is that visual features from sparse
% % clips already capture key visual and semantic information
% % in the video, as consecutive clips usually contain similar
% % semantics from a continuous scene. Thus, a handful of
% % clips are sufficient for training, instead of using the full
% % video.
% \textit{ii) Sparse temporal sampling:} 
% sparse video clips are already sufficient to capture key semantics for pre-training~\cite{lei2021less}.
% % only a single or a few sparsely sampled short clips from a video are used during pre-training. 
% % Recent end-to-end methods~\cite{Bain_2021_ICCV,lei2021less} adopt such strategy to accelerate pre-training.
% % ClipBERT~\cite{lei2021less} introduces a sparse temporal sampling strategy to remove redundant temporal information, which only samples one frame per video during pre-training.
% The core idea behind the above methods is removing visual redundancy. 
% Data reduction attempts to filter out useless noisy data and sparse temporal sampling tries to remove redundant temporal information from videos.

Towards this end, we further propose to remove the redundant spatial information in sparsely sampled video clips via the claim that \textit{a frame is actually worth around 30 objects} (based our experiments in Section~\ref{ablation}).
% In this work, we further attempt to remove redundant spatial information in videos.
Specifically, we revitalize offline region features that were all the rage in image-language tasks~\cite{lee2018stacked,liu2019focus} to encourage efficient VLP.
Region features are generally pre-extracted by a pre-learned object detector~\cite{anderson2018bottom}.
Rather than the dense and continuous visual signal of the raw pixels, the region features are sparsely distributed with the compact information of salient visual contents, which are the most useful for video-text understanding.
We further advocate ``\textit{less is more}'' for one more step towards democratizing VLP research.
% They are sparsely distributed in a frame and only focus on objects and salient visual contents.
% Less important spatial information, such as the background, is ignored.
% They focus on objects and salient visual contents that are multi-scale regions and sparsely distributed in image.
% Because the number of objects and events that appear in a video is limited, we only need to sample a small number of region features to represent a video.
% Thus, the pre-training period is accelerated sharply.


% 3. (other loss not work well, how to use region feature (model, loss), video attributes -> not work, our loss specific to video) however, previous offline feature methods bad performance -> assumption: 1. tasks disconnection; 2. modality disconnection -> action recognition bad, object detection good; our alignment cope with modality disconnection -> generalization to different models
As is known, methods using off-the-shelf features~\cite{lee2018stacked,liu2019focus} have been phased out in visual-language tasks due to the inferior downstream performances.
% However, such offline-extracted video features are gradually being phased out of VLP because of the poor performance on downstream tasks.
Previous work~\cite{lei2021less} attributes the unsatisfactory pre-training performance of pre-extracted features to their disconnections with the current domain and language modality. 
We would like to clarify that such disconnections can be properly eliminated by imposing fine-grained cross-modality alignment regularization.

Specifically, besides the common late fusion regularization on the global visual-text representations \cite{Bain_2021_ICCV}, 
% offline feature extractor are often trained for pre-tasks (e.g., action recognition~\cite{feichtenhofer2019slowfast,hara2018can}) which are different from VLP, and we cannot finetune the offline feature during pre-training.
% Such disconnection between pre-tasks and VLP makes offline video features are hard to align with language.
% Meanwhile, the most existing methods~\cite{Bain_2021_ICCV,lei2021less,zhu2020actbert,luo2020univl} connect video and language with simple alignment methods, which also makes offline features perform poorly.
% They either maximize the cosine similarity of a video and language feature~\cite{Bain_2021_ICCV}, or use a fused feature of video and language to perform binary classification~\cite{lee2018stacked,zhu2020actbert,luo2020univl}.
% These coarse-grained alignment methods miss detailed information in both video and text. 
% Meanwhile, a simple contrastive loss, which is adopted by most VLP methods, between video and textual features is not enough to build a 
% \textit{i) Tasks disconnection :} offline feature extractors are often trained on tasks, e.g., action recognition~\cite{feichtenhofer2019slowfast,hara2018can}, that are different from video-language tasks. 
% \textit{ii) Modality disconnection:} offline features from different modalities are independent from each other.
% It is hard to build a connection between different modalities. 
% To better align video with language, 
we introduce a novel bidirectional region-word alignment regularization under the observation that
% exploring more details.
% We find that the the video-language tasks indeed have the disconnection with action recognition, whereas region features adapt well with them.
% We observe that 
% objects and attended regions in video frames are naturally related to some words in a sentence.
objects extracted from video frames are naturally associated with certain words in the corresponding sentences.
%
For instance, as demonstrated in Fig.~\ref{fig:intro}, the keywords ``people", ``car" and ``bicycle" share high-level semantics with cropped regions (highlighted with bounding boxes), respectively.
To model and promote such a detailed cross-modality relationship, we build bidirectional connections between extracted regions and words.
% We estimate fine-grained region-to-word and word-to-region attention weights
In the \texttt{Region$\rightarrow$Word} manner, 
we estimate the region-to-sentence similarity resorting to the similarities between each region and all the words in a sentence.
% (1) estimate region-to-word cosine similarities for each region;
% (2) build the attention weights via normalizing the similarities with a softmax operation;
% (3) ensemble the word features into a sentence feature according to the attention weights;
% (4) estimate the region-to-sentence similarity by computing the cosine similarity between the region feature and the ensembled sentence feature.
% pick the most relevant word for each region feature to construct a region-word pair according to the attention weights which are estimated by the cosine similarities.
% region features attend to words in a sentence, and then the most relevant words are picked up according to attention weights.
% Each region and its corresponding words are used to compute similarity.
The average region-to-sentence similarity over all the regions of a video clip is treated as the video-to-sentence similarity, which is further maximized for positive pairs.
Similarly, the \texttt{Word$\rightarrow$Region} manner is conducted to measure and optimize the sentence-to-video similarity according to the similarities between each word and the corresponding regions.
% attend to regions with respect to words and compute language-to-video similarity.
% By maximizing video-to-language and language-to-video similarities, the region-word alignment is built up. 
We surprisingly find that the proposed fine-grained region-word alignment constraints can also be seamlessly integrated into end-to-end VLP methods \cite{Bain_2021_ICCV}, achieving promising performance gains.
% Another advantage is that the proposed alignment can seamlessly adapt with other end-to-end VLP methods.
% Such fine-grained alignment also improves other VLP methods.
% Empirical results in previous image-language pre-training models~\cite{li2020oscar,chen2020uniter} also verify that region features are suitable for visual-language tasks.

% loss generalization


% contributions: 1. vlp model efficient; 2. new loss to better align video-text; 3. sota experimental results 4. democratize (bonus)

% 2. faces problems: 1) require massive data->cost a lot of pre-training time; 2) lack a strong fine-grained alignment between video-language；现有的方法需要大量的数据和很长的pretrain时间，不论是offline还是e2e的方法；同时，由于Transformer backbone和处理video已经占用了大量的计算资源和显存，缺乏对于video-language的fine-grained alignment设计。
% Although these methods have achieved significant progress, they still suffer from the requirement of massive pre-training data and long pre-training time. 
% Because the model capacity of VLP models is typically large, the most commonly used dataset is HowTo100M~\cite{miech2019howto100m}. 
% As recent high-quality datasets proposed, such as WebVid2.5M~\cite{Bain_2021_ICCV}, the needed amount of pre-training data is reduced to less than 10 million, which is still very large.
% Besides large-scale dataset, high computational cost also makes VLP models inefficient.
% Specifically, two main factors cause high computational cost: \textit{i) dense frames per video :} multiple frames per video are sampled to extract representations. \textit{ii) dense grids per frame:} each video frame is represented by hundreds of feature vectors. For example, if ResNet~\cite{he2016deep} is used as the video encoder, the last-layer feature map is reshaped to 144 vectors to represent the frame.
% Due to self-attention in Transformer is $O(N)^2$ time complexity, such dense grids lower efficiency heavily.
% Even the most efficient framework, ClipBERT~\cite{lei2021less}, requires 768 GPU hours to finish the pre-training.

% Another side effect caused by such a high-computational-cost framework is that exploration of video-language alignment is limited.
% % To learn join video-language representations, video-language alignment performs a key role, because the aligned multi-modal representations with the same semantics are the foundation of downstream video-language tasks.
% Transformer-based modules and video processing in VLP methods~\cite{dosovitskiy2020vit,bertasius2021space} have already consumed large computation resources and GPU memory.
% Thus, existing methods~\cite{Bain_2021_ICCV,lei2021less,zhu2020actbert,luo2020univl} tend to connect video and language with simple alignment methods.
% They either maximize the cosine similarity of a video and language feature~\cite{Bain_2021_ICCV}, or use a fused feature of video and language to perform binary classification~\cite{lee2018stacked,zhu2020actbert,luo2020univl}.
% These global alignment methods miss the fine-grained connection between regions and words.

% 3. by introducing object-feature, we democratize video-language pre-training: 1) fewer feature vectors to represent a video frame; 2) less data for pre-training; such fast pre-training enables us to propose a fine-grained region-word alignment; region-word alignment can be easily extended to other pre-training framework.为了解决上述两个问题，我们引入了object region feature来democratize VLP。object feature有几个好处：1）2）3）。由于计算资源大大减少，我们可以设计更为复杂和fine-grained的alignment。本文，我们通过建立region-word alignment和video-sentence alignment，从global和local两个层次连接video和language
% To solve the above issues, we democratize video-language pre-training by introducing region features to save pre-training time and propose a fine-grained video-language alignment to better connect video and language. 
% Specifically, we revitalize region features that have been widely used in image-language tasks and image-language pre-training~\cite{chen2020uniter,li2020oscar} to reach efficient VLP. 
% Region features are extracted by a pre-trained object detector~\cite{anderson2018bottom} to represent videos.
% Different from feature maps of CNNs~\cite{he2016deep,huang2017densely} or patch embeddings of ViT~\cite{dosovitskiy2020vit} that correspond to dense and uniform grids of equally sized image patches, region features focus on objects and salient visual contents that are multi-scale regions and sparsely distributed in images.
% Because the number of objects and events that appear in a video is limited, we only need to sample a small number of region features to represent a video.
% Thus, the pre-training period is accelerated sharply.

% To better connect video and language, we propose a novel global-local video-language alignment based on region features.
% The global alignment follows previous coarse-grained methods~\cite{Bain_2021_ICCV}.
% The dot product of video and language feature vectors is maximized to align a pair of video and caption.
% The local alignment builds bidirectional connections between regions and words.
% In the \texttt{Region$\rightarrow$Word} manner, region features attend to words in a sentence, and then the most relevant words are picked up according to attention weights.
% Each region and its corresponding words are used to compute similarity.
% The average similarity over regions is the video-to-language similarity.
% Similarly, the \texttt{Word$\rightarrow$Region} manner is conducted to attend to regions with respect to words and compute language-to-video similarity.
% By maximizing video-to-language and language-to-video similarities, the local alignment is built up.

In summary, our contributions are three-fold:
\begin{itemize}
    \item We revitalize region features towards democratizing VLP via removing both temporal and spatial visual redundancy.
    % reach efficient pre-training. 
    Specifically, our efficient VLP model can maintain state-of-the-art performance on multiple downstream tasks with 80\% fewer data and 85\% less pre-training time than ClipBERT~\cite{lei2021less}, which is the most efficient end-to-end VLP method so far. 
    % compared to recent dominant end-to-end methods \cite{Bain_2021_ICCV,lei2021less}.
    \item We clarify that the inferior performance of off-the-shelf features in previous attempts \cite{li2020hero,zhu2020actbert,sun2019videobert,yu2018joint,gabeur2020multi} lies in the sub-optimal learning regularization. We tackle the challenge with a newly proposed bidirectional region-word constraint, which optimizes fine-grained visual-text relations and properly eliminates the domain/modality disconnections of the region features.
    % propose a region-word alignment to connect video and language in a fine-grained way. It can generalize to other VLP methods.
    \item Our method shows competitive results on seven downstream tasks, including video-to-text retrieval and video question answering.
    % spanning finetuning and zero-shot transfer. 
    We surprisingly observe that the introduced region-word alignment regularization can also effectively boost the end-to-end method \cite{Bain_2021_ICCV} with noticeable improvements.
    % Comprehensive ablation studies demonstrate the key factors that lead to powerful and efficient video-language pre-training.
\end{itemize}

==> sections/1-Intro.tex <==
\section{Introduction}
% 1. vlp发展，用于很多vl tasks；e2e方法dominate，但pretrain需要大量数据，并十分耗时，许多researcher难以展开vlp研究；democratization包括两方面：1. efficient 2. generality
% 2. efficient: clean data可以达到小规模数据，效果更佳->同理，raw image有噪声信息，region feature有更多有效信息->clipbert指出modality 和task的disconnection导致offline feature效果不佳->我们认为效果不佳的原因是用的方法不对，我们的loss如何解决了这两个disconnection
% 3. generality: real democratize需要我们方法上的strategy同样可以generalize到e2e的方法上；empirical study证明我们的loss可以适用于e2e patch方法和e2e region方法；
% contribution: 1 democratize vlp model; efficient; 2. new loss to better align video-text; 3. sota experimental results

% 1. video-language pre有更多有效信息；-training； VLP发展，可以用于很多downstream tasks；e2e方法dominated，但是十分耗时，许多researcher难以开展vlp研究
% Video-language tasks, such as text-to-video retrieval~\cite{lee2018stacked,liu2019focus}, video question answer~\cite{anderson2018bottom} and video caption~\cite{anderson2018bottom,sharma2018conceptual}, require joint learning of video and language representations. 
% Recently, video-language pre-training (VLP)~\cite{Bain_2021_ICCV,lei2021less,li2020hero,miech2020end} that follows the pre-training-and-finetune scheme has become the most popular practice to cope with these tasks.
Video-Language pre-training (VLP)~~\cite{Bain_2021_ICCV,lei2021less,li2020hero,miech2020end} that jointly learns video and language representations in a self-supervised manner has become the most popular practice to cope with video-language tasks, such as text-to-video retrieval~\cite{lee2018stacked,liu2019focus}, video question answer~\cite{anderson2018bottom} and video caption~\cite{anderson2018bottom,sharma2018conceptual}.
% The typical paradigm of existing VLP approaches is to extract video and language features and then fuse them to learn a join video-language representations. 
% Generally, the textual encoder and fusion module is based on Transformer~\cite{vaswani2017attention}.
% As for the video encoder, most VLP methods~\cite{li2020hero,yu2018joint,gabeur2020multi,zhu2020actbert} utilize pre-trained action recognition models~\cite{feichtenhofer2019slowfast,hara2018can} to extract video features. 
% Recent methods~\cite{Bain_2021_ICCV,lei2021less,zellersluhessel2021merlot} attempt to develop end-to-end VLP models that learn video representation from raw pixels.
Recently, end-to-end methods~\cite{Bain_2021_ICCV,lei2021less,zellersluhessel2021merlot} that learn video representations from raw pixels have been dominated because of their strong performance on downstream task.
However, they still suffer from the requirement of massive pre-training data and long pre-training time, which causes many researcher hard to pursue research in VLP.

% 2. existing methods tries to democratize VLP: 1. high-quality data; 2. temporal sparse sampling. ->core idea: remove noisy data -> region, spatial sparse sampling -> revitalize region features in previous image-text tasks -> accelerate pre-training
Existing methods~\cite{Bain_2021_ICCV,lei2021less} have explored efficient VLP models from two perspectives: 
\textit{i) Data reduction:} a clean dataset can sharply reduce the needed amount of pre-training data.
For example, Frozen~\cite{Bain_2021_ICCV} proposes a high-quality dataset, WebVid2.5M to replace the most common used dataset, HowTo100M~\cite{miech2019howto100m}.
% Compared with the large-scale noisy datasets, a clean dataset reduces the needed amount of pre-training data to less than 10 million.
\textit{i) Sparse temporal sampling:} only a single or a few sparsely sampled short clips from a video are used during pre-training. 
Recent end-to-end methods~\cite{Bain_2021_ICCV,lei2021less} adopt such strategy to accelerate pre-training.
% ClipBERT~\cite{lei2021less} introduces a sparse temporal sampling strategy to remove redundant temporal information, which only samples one frame per video during pre-training.
The core idea behind above methods is removing redundant data. 
Data reduction attempts to filter out useless noisy data and sparse temporal sampling tries to remove redundant temporal information from videos.

In this work, we further attempt to remove redundant spatial information in videos.
Specifically, we revitalize region features that have been widely used in image-language tasks~\cite{lee2018stacked,liu2019focus} to reach efficient VLP.
Region features are extracted by a pre-trained object detector~\cite{anderson2018bottom} from each frame.
They are sparsely distributed in a frame and only focus on objects and salient visual contents.
Less important spatial information, such as the background, is ignored.
% They focus on objects and salient visual contents that are multi-scale regions and sparsely distributed in image.
Because the number of objects and events that appear in a video is limited, we only need to sample a small number of region features to represent a video.
Thus, the pre-training period is accelerated sharply.

% 3. (other loss not work well, how to use region feature (model, loss), video attributes -> not work, our loss specific to video) however, previous offline feature methods bad performance -> assumption: 1. tasks disconnection; 2. modality disconnection -> action recognition bad, object detection good; our alignment cope with modality disconnection -> generalization to different models
However, such offline-extracted video features are gradually being phased out of VLP because of the poor performance on downstream tasks.
Previous work~\cite{lei2021less} ascribes the inferior performance to a reason that offline feature extractor are often trained for pre-tasks (e.g., action recognition~\cite{feichtenhofer2019slowfast,hara2018can}) which are different from VLP, and we cannot finetune the offline feature during pre-training.
Such disconnection between pre-tasks and VLP makes offline video features are hard to align with language.
Meanwhile, the most existing methods~\cite{Bain_2021_ICCV,lei2021less,zhu2020actbert,luo2020univl} connect video and language with simple alignment methods, which also makes offline features perform poorly.
They either maximize the cosine similarity of a video and language feature~\cite{Bain_2021_ICCV}, or use a fused feature of video and language to perform binary classification~\cite{lee2018stacked,zhu2020actbert,luo2020univl}.
These coarse-grained alignment methods miss detailed information in both video and text. 
% Meanwhile, a simple contrastive loss, which is adopted by most VLP methods, between video and textual features is not enough to build a 
% \textit{i) Tasks disconnection :} offline feature extractors are often trained on tasks, e.g., action recognition~\cite{feichtenhofer2019slowfast,hara2018can}, that are different from video-language tasks. 
% \textit{ii) Modality disconnection:} offline features from different modalities are independent from each other.
% It is hard to build a connection between different modalities. 

To better align video with language, we propose a novel region-word alignment to exploring more details.
% We find that the the video-language tasks indeed have the disconnection with action recognition, whereas region features adapt well with them.
We observe that objects and attended regions in video frames are naturally related to some words in a sentence.
For example, as shown in Fig.~\ref{fig:framework}, the words ``woman", ``man" and ``lamp" share the same semantics with regions (highlighted with bounding boxes).
To model such detailed relationship, we builds bidirectional connections between regions and words.
In the \texttt{Region$\rightarrow$Word} manner, region features attend to words in a sentence, and then the most relevant words are picked up according to attention weights.
Each region and its corresponding words are used to compute similarity.
The average similarity over regions is the video-to-language similarity.
Similarly, the \texttt{Word$\rightarrow$Region} manner is conducted to attend to regions with respect to words and compute language-to-video similarity.
By maximizing video-to-language and language-to-video similarities, the region-word alignment is built up. 
Another advantage is that the proposed alignment can seamlessly adapt with other end-to-end VLP methods.
Such fine-grained alignment also improves other VLP methods.
% Empirical results in previous image-language pre-training models~\cite{li2020oscar,chen2020uniter} also verify that region features are suitable for visual-language tasks.

% loss generalization


% contributions: 1. vlp model efficient; 2. new loss to better align video-text; 3. sota experimental results 4. democratize (bonus)

% 2. faces problems: 1) require massive data->cost a lot of pre-training time; 2) lack a strong fine-grained alignment between video-language；现有的方法需要大量的数据和很长的pretrain时间，不论是offline还是e2e的方法；同时，由于Transformer backbone和处理video已经占用了大量的计算资源和显存，缺乏对于video-language的fine-grained alignment设计。
% Although these methods have achieved significant progress, they still suffer from the requirement of massive pre-training data and long pre-training time. 
% Because the model capacity of VLP models is typically large, the most commonly used dataset is HowTo100M~\cite{miech2019howto100m}. 
% As recent high-quality datasets proposed, such as WebVid2.5M~\cite{Bain_2021_ICCV}, the needed amount of pre-training data is reduced to less than 10 million, which is still very large.
% Besides large-scale dataset, high computational cost also makes VLP models inefficient.
% Specifically, two main factors cause high computational cost: \textit{i) dense frames per video :} multiple frames per video are sampled to extract representations. \textit{ii) dense grids per frame:} each video frame is represented by hundreds of feature vectors. For example, if ResNet~\cite{he2016deep} is used as the video encoder, the last-layer feature map is reshaped to 144 vectors to represent the frame.
% Due to self-attention in Transformer is $O(N)^2$ time complexity, such dense grids lower efficiency heavily.
% Even the most efficient framework, ClipBERT~\cite{lei2021less}, requires 768 GPU hours to finish the pre-training.

% Another side effect caused by such a high-computational-cost framework is that exploration of video-language alignment is limited.
% % To learn join video-language representations, video-language alignment performs a key role, because the aligned multi-modal representations with the same semantics are the foundation of downstream video-language tasks.
% Transformer-based modules and video processing in VLP methods~\cite{dosovitskiy2020vit,bertasius2021space} have already consumed large computation resources and GPU memory.
% Thus, existing methods~\cite{Bain_2021_ICCV,lei2021less,zhu2020actbert,luo2020univl} tend to connect video and language with simple alignment methods.
% They either maximize the cosine similarity of a video and language feature~\cite{Bain_2021_ICCV}, or use a fused feature of video and language to perform binary classification~\cite{lee2018stacked,zhu2020actbert,luo2020univl}.
% These global alignment methods miss the fine-grained connection between regions and words.

% 3. by introducing object-feature, we democratize video-language pre-training: 1) fewer feature vectors to represent a video frame; 2) less data for pre-training; such fast pre-training enables us to propose a fine-grained region-word alignment; region-word alignment can be easily extended to other pre-training framework.为了解决上述两个问题，我们引入了object region feature来democratize VLP。object feature有几个好处：1）2）3）。由于计算资源大大减少，我们可以设计更为复杂和fine-grained的alignment。本文，我们通过建立region-word alignment和video-sentence alignment，从global和local两个层次连接video和language
% To solve the above issues, we democratize video-language pre-training by introducing region features to save pre-training time and propose a fine-grained video-language alignment to better connect video and language. 
% Specifically, we revitalize region features that have been widely used in image-language tasks and image-language pre-training~\cite{chen2020uniter,li2020oscar} to reach efficient VLP. 
% Region features are extracted by a pre-trained object detector~\cite{anderson2018bottom} to represent videos.
% Different from feature maps of CNNs~\cite{he2016deep,huang2017densely} or patch embeddings of ViT~\cite{dosovitskiy2020vit} that correspond to dense and uniform grids of equally sized image patches, region features focus on objects and salient visual contents that are multi-scale regions and sparsely distributed in images.
% Because the number of objects and events that appear in a video is limited, we only need to sample a small number of region features to represent a video.
% Thus, the pre-training period is accelerated sharply.

% To better connect video and language, we propose a novel global-local video-language alignment based on region features.
% The global alignment follows previous coarse-grained methods~\cite{Bain_2021_ICCV}.
% The dot product of video and language feature vectors is maximized to align a pair of video and caption.
% The local alignment builds bidirectional connections between regions and words.
% In the \texttt{Region$\rightarrow$Word} manner, region features attend to words in a sentence, and then the most relevant words are picked up according to attention weights.
% Each region and its corresponding words are used to compute similarity.
% The average similarity over regions is the video-to-language similarity.
% Similarly, the \texttt{Word$\rightarrow$Region} manner is conducted to attend to regions with respect to words and compute language-to-video similarity.
% By maximizing video-to-language and language-to-video similarities, the local alignment is built up.

In summary, our main contributions are:
\begin{itemize}
    \item We revitalize region features in video-language pre-training to reach efficient pre-training. Our most efficient model can hold state-of-the-art results on downstream tasks even when reducing 80\% data and 75\% pre-training time.
    \item We propose a region-word alignment to connect video and language in a fine-grained way. It can generalize to other VLP methods.
    \item Our method shows competitive results on 7 downstream tasks, spanning finetuning and zero-shot transfer. Comprehensive ablation studies demonstrate the key factors that lead to powerful and efficient video-language pre-training.
\end{itemize}

==> sections/2-Related.tex <==
\section{Related Work}

\noindent\textbf{Video-Language Pre-training.}
% Massive video-language pairs on the Internet encourage the research on large-scale video-language pre-training (VLP). 
% VLP models have shown remarkable performance on different video-language tasks, such as video-language retrieval~\cite{Bain_2021_ICCV,gabeur2020multi,wang2021dig,yu2018joint}, video question answering~\cite{Yang_2021_ICCV} and video caption~\cite{luo2020univl}. 
% offline, action-recognition backbone
Early VLP methods~\cite{li2020hero,zhu2020actbert,sun2019videobert,yu2018joint,gabeur2020multi,wang2021dig} introduce pretrained models on other tasks to pre-extract video representations.
Some of them~\cite{li2020hero,zhu2020actbert,sun2019videobert} utilize action recognition backbones~\cite{feichtenhofer2019slowfast,hara2018can} to pre-extract video representations.
These backbones are designed with 2D~\cite{he2016deep} and 3D~\cite{hara2018can} CNNs to capture spatial and temporal information in videos. 
Others~\cite{yu2018joint,liu2019use,gabeur2020multi,wang2021dig} fuse multiple ``Experts" that are trained on different modalities, such as audio classification~\cite{hershey2017cnn}, OCR~\cite{gabeur2020multi}, image classification~\cite{huang2017densely} and so on, to fully exploit cross-modal high-level semantics in videos.
% e2e, (vit, cnn)
Recently, end-to-end models~\cite{miech2020end,lei2021less,Bain_2021_ICCV,zellersluhessel2021merlot,fu2021violet} are proposed .
Some~\cite{miech2020end,lei2021less,zellersluhessel2021merlot} utilize CNNs to extract video features, others~\cite{Bain_2021_ICCV,fu2021violet} replace CNNs with ViT~\cite{dosovitskiy2020vit} to build a pure Transformer-based VLP model.
% MIL-NCE~\cite{miech2020end}, ClipBERT~\cite{lei2021less} and MERLOT~\cite{zellersluhessel2021merlot} utilize CNNs to extract video features. 
% Frozen~\cite{Bain_2021_ICCV} and VIOLET~\cite{fu2021violet} replace CNNs with ViT~\cite{dosovitskiy2020vit} to build a pure Transformer-based VLP model.

\noindent\textbf{Region Features in Image-Language Pre-training.}
% object feature
Region features extracted by an object detector~\cite{anderson2018bottom} are adopted by image-language pre-training (ILP) methods~\cite{chen2020uniter,li2020oscar}.
They represent an image to a set of region features that focus on salient regions that are a much more natural basis for attention~\cite{egly1994shifting,scholl2001objects}.
Region features enable the interaction between image and text at the object level.
Recent ITP methods~\cite{li2020oscar,chen2020uniter,yao2022filip} attempt to form fine-grained alignment between image and text based on region features.  

% Many image-language pre-training models adopt region features extracted by an object detector~\cite{anderson2018bottom} to represent images, because region features focus on salient regions that are a much more natural basis for attention~\cite{egly1994shifting,scholl2001objects}.
% However, only ActBERT~\cite{zhu2020actbert} explores it in VLP. 
% In this work, we rethink region features for VLP and use them to democratize VLP in an efficient way.

\noindent\textbf{Fine-Grained Alignment between Vision and Language.} 
Fine-grained alignment between visual and textual contents has been explored in image-language retrieval for several years. 
% The coarse-grained alignment~\cite{wang2018learning,zhang2018deep} attempts to maximize the cosine similarity of a whole image and sentence. 
% To achieve fine-grained alignment, some works~\cite{lee2018stacked,liu2019focus,li2017identity,chen2020fine,wang2019camp,yao2022filip} propose different attention mechanisms to match visual regions and captions.
Some studies~\cite{lee2018stacked,liu2019focus,li2017identity,chen2020fine,wang2019camp,yao2022filip} propose different attention mechanisms to match visual regions and captions.
Recent ITP methods~\cite{li2020oscar,chen2020uniter} also explore the alignment between regions and words.
% However, due to the complex attention mechanism, such fine-grained alignment lacks efficiency and requires large GPU memory consumption. 
Considering the low efficiency and large GPU memory consumption for video processing, previous VLP methods~\cite{luo2020univl,sun2019videobert,rouditchenko2021cascaded,gabeur2020multi} adopt simple contrastive loss or binary classification to align video and language.
Recently, TACo~\cite{yang2021taco} has attempted to build up a fine-grained alignment.
However, it still suffers from so large computation cost that simplifies its original design.
In this work, benefitting from our efficient pipeline, we propose a novel region-word alignment method to better connect the video and language.

% In video-language pre-training, considering the Transformer-based backbone and video processing also requires large computation cost and GPU memory consumption, fine-grained alignment is hardly adopted. 
% Recently, TACo~\cite{yang2021taco} has attempted to build up a fine-grained alignment.
% However, it still suffers from so large computation cost that simplifies its original design.
% In this work, benefitting from our efficient pipeline, we propose a novel region-word alignment method to better connect the video and language.

==> sections/3-Method.tex <==
\input{figs/framework}
\section{Method}

The framework of our method is illustrated in Fig.~\ref{fig:framework}. A video and its corresponding caption are taken as input. 
The video is initially embedded to region features by an off-the-shelf object detector~\cite{anderson2018bottom} before being fed into a video encoder. 
The corresponding caption is encoded to language features by a language encoder. 
During the pre-training, the video and caption features are optimized towards the objective of global-local alignment. 
% To ensure efficiency, we only sample one frame per video and a small number of regions per frame. 
After pre-training, the model can be transferred to a variety of downstream video-language tasks with fine-tuning.
% \input{figs/framework}

\subsection{Model Architecture.}

\noindent\textbf{Input.} 
% Our method takes paired video $V$ and sentence $T$ as inputs. Video frames $\{f_1, f_2, ...\}$ are sampled from $V$. 
% They are processed to region features $\{r_0, r_1, r_2, ...\}$ by video encoder. 
% Word tokens $\{w_0, w_1, w_2, ...\}$ from $T$ are processed by language encoder to language features $\{t_0, t_1, t_2, ...\}$.
Our method takes paired video $V$ and sentence $T$ as raw inputs. 
Similar to previous VLP methods~\cite{Bain_2021_ICCV,lei2021less}, $T$ is tokenized into word tokens $\{w_l\}^{L}_{l=0}$, where $L$ denotes the number of tokens in $T$ and $w_0$ denotes the [CLS] token. 
These word tokens are inputted to language encoder.
Video frames $\{f_1, f_2, ..., f_M\}$ are sampled from $V$, where $M$ denotes the number of frames.  
Given frames $\{f_1, f_2, ..., f_M\}$ of a video, objects and salient regions in each frame are detected by Faster RCNN~\cite{anderson2018bottom} pre-trained on Visual Genome~\cite{krishna2017visual}. 
Pooled RoI features of these regions are concatenated together as features $\{o_n\in \mathbb{R}^d\}^{N}_{n=1}$ of the whole video, where $N$ denotes the number of regions.
Video encoder takes these RoI features as the inputs.

In this work, we use pre-extracted region features rather than fine-tuning the detector end-to-end for efficient pre-training. Tuning the detector requires extra computational and memory overhead, and it is also infeasible to acquire bounding box annotations in video-language datasets.
% , because it increases the computation cost and the ground-truth annotation is inaccessible.

% 2 component, 重点介绍第一部分变成region feature的好处，具体使用的detector引用和公式即可；第二部分ViT也可以简单介绍 
\noindent\textbf{Video Encoder.} 
% Video encoder consists of an object detector~\cite{anderson2018bottom} to extract region features and a ViT~\cite{dosovitskiy2020vit} to refine them. 
% Given frames $\{f_1, f_2, ...\}$ of a video, objects and salient regions in each frame are detected by the detector. 
% RoI features of these regions are concatenated together as region features $\{o_n\}^{N}_{n=1}$ of the whole video, where $N$ denotes the number of regions.
We add a [CLS] token $o_0$ to represent the whole video so that the input becomes $\{o_n\}^{N}_{n=0}$.
To encode location information for each region feature, we use a linear layer $FC$ to project 7-dimensional location vectors $\{l_n=[x_1, y_1, x_2, y_2, w, h, w*h]\}^{N}_{n=0}$ (normalized top/left/bottom/right coordinates, width, height and area) to $\{l_n^\prime \in \mathbb{R}^d\}^N_{n=0}$:
\begin{equation}
    l_n^\prime = FC(l_n)
\end{equation}
Learned temporal position embeddings $\textbf{P}\in \mathbb{R}^{M\times d}$ are used to model temporal clues.
% After adding a [CLS] token, $o_0$, to original region features, $\{o_n\}^{N}_{n=1}$ are refined by ViT: $\{r_n\}^{N}_{n=0} = ViT(\{o_n\}^{N}_{n=0})$, where $r_n$ denotes the refined region feature. 
Video Encoder encodes $\{o_n\}^{N}_{n=0}$ with a Transformer-based network $E_V$:
\begin{equation}
    \{r_n\}^{N}_{n=0} = E_V(\{o_n+l_n^\prime+\textbf{P}_m\}^{N}_{n=0})
\end{equation}
where $r_n$ denotes the output region feature, and $m$ denotes $o_n$ is extracted from $m$-th frame.
We introduce ViT~\cite{dosovitskiy2020vit} as $E_V$.
% $l_n$ denotes the location vector and $E_V$ is a Transformer-based network.
% $E_V$ is a Transformer-based network.
% To encoder location information for each region feature, we use a linear layer $FC$ to project 7-dimensional location vectors $\{l_n=[x_1, y_1, x_2, y_2, w, h, w*h]\}^{N}_{n=0}$ (normalized top/left/bottom/right coordinates, width, height and area) to the same feature space with $o_n$.
Video Encoder makes region features interplay with each other, and outputs refined region features $\{r_n\}^{N}_{n=0}$, where $r_0$ is encoded from [CLS] token and treated as the global video feature. 
% The region features is obtained by summing up the location feature and RoI features, denoted as $\{o^\prime_n\}^{N}_{n=1}$.
% Video Encoder (VE) takes the region features as input and establish relationships between region features, the video encoder (VE) processes them to refined region features: $\{r_n\}^{N}_{n=0} = VE(\{o_n\}^{N}_{n=0})$, where $r_n$ denotes the refined region feature.
% 简单介绍text怎么处理，使用distillbert，公式介绍，效率方面的优势

\noindent\textbf{Language Encoder.} 
% Similar to previous VLP methods~\cite{lei2021less,Bain_2021_ICCV}, the language input $T$ is tokenized into word tokens $\{w_l\}^{L}_{l=0}$, where $L$ denotes the number of tokens in $T$ and $w_0$ denotes the [CLS] token. 
% Similarly, the language encoder (LE) embeds each word token $w_l$ into language feature $t_l$: $\{t_l\}^{L}_{l=0} = LE(\{w_l\}^{L}_{l=0})$. 
% Specifically, to improve efficiency, we adopt DistillBERT~\cite{sanh2019distilbert} as LE, which has 40\% less parameters than BERT~\cite{devlin2018bert} and preserves over 95\% of BERT's performance.
Similar to previous VLP methods~\cite{lei2021less,Bain_2021_ICCV}, Language Encoder is based on BERT~\cite{devlin2018bert}. Word tokens are encoded to $\{t_l\in\mathbb{R}^d\}^L_{l=0}$:
\begin{equation}
    \{t_l\}^{L}_{l=0} = E_V(\{w_l\}^{L}_{l=0})
\end{equation}
where $t_l$ denotes the output language feature and we adopt DistillBERT~\cite{sanh2019distilbert} as $E_L$, which has 40\% less parameters than BERT~\cite{devlin2018bert} and preserves over 95\% of BERT's performance.
The outputs of Language Encoder $\{t_l\}^{L}_{l=0}$ are then aligned with region features by our proposed pre-training objective.

\subsection{Reduce Visual Redundancy.}
To democratize video-language pre-training, we attempt to remove both temporal and spatial redundancy.
We involve two training strategies to ensure the pre-training time is acceptable.

\noindent\textbf{Temporal Visual Redundancy - Frame Sparse Sampling.}
To save pre-training time and reduce GPU memory consumption, we adopt a sparse frame sapling strategy similar to ClipBERT~\cite{lei2021less}. 
During the pre-training period, only a single frame is sampled randomly for each video. 
When finetuning on downstream tasks, a dense sampling strategy is adopted to capture more visual information from videos. 
We observe that such extremely sparse sampling still achieves competing results on downstream tasks in our framework.

\noindent\textbf{Spatial Visual Redundancy - Object Region Extraction.}
Considering the number of objects and salient regions detected by an object detector is uncertain, to balance the efficiency and performance, we tend to extract 30 region features per frame (we observe that 30 regions are enough for VLP according to our experiments in Section~\ref{ablation}).
We explore two selection strategies: \textbf{i) Sorted Selection}. 
Top 30 regions with the highest detection confidence are selected. 
We attempt to choose the most discriminative region features with this strategy. 
\textbf{ii) Track Object}. 
We conduct object tracking to form a tracklet for each object. 
Only one region feature is reserved for each tracklet.
We attempt to remove redundant objects that repeat in continuous frames to cover more object categories with this strategy.
In default, we perform sorted selection.
% Meanwhile, to find the most salient regions and avoid noisy data, we choose the top 30 regions with respect to the detection confidence. 
% The regions with higher confidence will be selected.
% If the number of detected regions in a frame is less than 30, we will pad zero vectors as region features.



\subsection{Pre-training Objective.}
To jointly learn video-language representations from large-scale datasets~\cite{Bain_2021_ICCV,miech2019howto100m}, we introduce a global-local video-language alignment to connect video and language from coarse to fine. 
The global-local alignment consists of two pre-training objectives: \textbf{i) video-sentence alignment}, and \textbf{ii) region-word alignment}. In detail, for video-sentence alignment, we employ contrastive learning~\cite{Bain_2021_ICCV} with [CLS] tokens to align video and language globally. 
In the region-word alignment, regions and words are aligned to reach fine-grained alignment via a newly proposed bidirectional regularization.

\noindent\textbf{Video-Sentence Alignment.} 
Two losses are optimized to increase the video-to-language and language-to-video similarity:
\begin{equation}
\small
    \mathcal{L}^{\text{global}}_{\text{v2l}}=-\frac{1}{B}\sum^{B}_{i}\log\frac{\exp(r_{\text{cls}}^{i^{T}}t_{\text{cls}}^{i}/\sigma)}{\sum^{B}_{j}\exp(r_{\text{cls}}^{i^{T}}t_{\text{cls}}^{j}/\sigma)}
\end{equation}
\begin{equation}
\small
    \mathcal{L}^{\text{global}}_{\text{l2v}}=-\frac{1}{B}\sum^{B}_{i}\log\frac{\exp(t_{\text{cls}}^{i^{T}}r_{\text{cls}}^{i}/\sigma)}{\sum^{B}_{j}\exp(t_{\text{cls}}^{i^{T}}r_{\text{cls}}^{j}/\sigma)}
\end{equation}
where $r_{\text{cls}}^i$ and $t_{\text{cls}}^j$ are normalized embeddings of $i$-th video's [CLS] token and $j$-th caption's [CLS] token in a batch of size $B$, respectively. 
$\sigma$ denotes the temperature coefficient.

\noindent\textbf{Region-Word Alignment.} 
The local alignment also attempts to maximize video-to-language and language-to-video similarity, but in a fine-grained way. 
We take video-to-language as an example to illustrate the details of region-word alignment. For $i$-th video with region features $\{r_n\}^{N}_{n=1}$ and $j$-th sentence with word features $\{t_l\}^{L}_{l=1}$, $n$-th region feature firstly attends to each word feature to pick up the most relevant words according to attention weights:
\begin{equation}
\small
    a_{n, l}=\frac{\exp(\langle r_n,t_l\rangle)}{\sum^{L}_{k=1}\exp(\langle r_n,t_k\rangle)}
\end{equation}
where $\langle \cdot,\cdot\rangle$ denotes the cosine similarity, $a_{n,l}$ denotes the similarity between the $n$-th region feature and $l$-th word feature. 
% 说避免noisy words这句话前面加个intuition，说一般只跟形容词、名词、动词关系大（cite几个用了名词动词做retrieval的paper），然后说其余的什么介词啥的就是没啥用，所以我们要用公式7去做refine
Intuitively, semantics in videos are usually associated with nouns, verbs and adjectives~\cite{yang2021taco,liu2019focus}.
Other types of words, e.g., prepositions, are not ``concrete" enough in videos~\cite{yang2021taco}.
Thus, to make the region only attend to the most relevant words and ignore other noisy words, we refine $a_{n,l}$ as follows:
\begin{equation}
\small
    a^\prime_{n,l}=\mathbbm{1}[a_{n,l} - \frac{1}{L}\sum^{L}_{k=1}a_{n,k}]\cdot a_{n,l}\label{eq:ref_attn}
\end{equation}
where $\mathbbm{1}[x]=1$ if $x>0$ else $0$. $a^\prime_{n,l}$ is the refined similarity between the $n$-th region feature and $l$-th word feature. Attention weights of irrelevant words are set to 0.
By conducting this operation, we ensure the model only focuses on the relevant words with respect to a video.

Given the similarity between region and word features, an attended sentence feature with respect to $n$-th region feature is calculated as follows:
\begin{equation}
\small
    \alpha_n = \sum^{L}_{l=1}a^\prime_{n,l}t_{l}
\end{equation}
where $\alpha_n$ denotes the attended sentence feature.
% Specifically, $[x_i/\sum^{N}_{i}x_i]_{+}=x_i/\sum^{N}_{i}x_i$ if $x_i>\frac{1}{N}\sum^{N}_{i}x_i$ else $[x_i/\sum^{N}_{i}x_i]_{+}=0$.
Thus, the similarity of $i$-th video and $j$-th caption can be computed as:  
\begin{equation}
\small
    S_{i,j}=\frac{1}{N}\sum^{N}_{n=1}\langle r_n, \alpha_{n}\rangle
\end{equation}
The video-to-language loss is calculated with contrastive loss:
\begin{equation}
\small
    % \mathcal{L}^{local}_{v2l}=\sum^{B}_{i=1}S_{i}log\frac{S_{i}}{q_{i}}\
    \mathcal{L}^{\text{local}}_{\text{v2l}}=-\frac{1}{B}\sum_{i}^B\log\frac{\exp(S_{i,i}/\sigma)}{\sum_{j}^B \exp(S_{i,j}/\sigma)}
\end{equation}
% where $S_i$ denotes a $B$-dimensional vector whose element is $S_{i,j}$, and $q_i$ denotes an one-hot vector where $q_{i,j}$ is $1$ if $i$-th video and $j$-th caption is a positive pair else $0$.
where $\sigma$ denotes the temperature coefficient.

The language-to-video loss $\mathcal{L}^{\text{local}}_{\text{l2v}}$ is calculated in the similar way as $\mathcal{L}^{\text{local}}_{\text{v2l}}$. Given the similarity $a_{l,n}$ between $l$-th word and $n$-th region, the attended video vector with respect to $l$-th word is calculated:
\begin{equation}
\small
    \beta_{l}=\sum^{N}_{n=1}\mathbbm{1}[a_{l,n} - \frac{1}{L}\sum^N_na_{l,n}]\cdot a_{l,n} \cdot r_{n}
\end{equation}
where $\beta_{l}$ denotes the attended video feature. 
The similarity of $j$-th caption and $i$-th video is:
\begin{equation}
\small
    S_{j,i}=\frac{1}{L}\sum^{L}_{l=1}\langle t_l, \beta_{l}\rangle
\end{equation}
The language-to-video loss $\mathcal{L}^{\text{local}}_{\text{l2v}}$ is then given as follows:
\begin{equation}
\small
    % \mathcal{L}^{local}_{l2v}=\sum^{B}_{j=1}S_{j}log\frac{S_{j}}{q_{j}}
    \mathcal{L}^{\text{local}}_{\text{l2v}}=-\frac{1}{B}\sum_{j}^B\log\frac{\exp(S_{j,j}/\sigma)}{\sum_{i}^B \exp(S_{j,i}/\sigma)}
\end{equation}

\noindent\textbf{Overall Pre-training Objective.} 
Combining the above four losses, the overall pre-training objective is:
\begin{equation}
\small
    \mathcal{L}=\mathcal{L}^{\text{global}}_{\text{v2l}}+\mathcal{L}^{\text{global}}_{\text{l2v}}+\mathcal{L}^{\text{local}}_{\text{v2l}}+\mathcal{L}^{\text{local}}_{\text{l2v}}
\end{equation}
% $\mathcal{L}=\mathcal{L}^{global}_{v2l}+\mathcal{L}^{global}_{l2v}+\mathcal{L}^{local}_{v2l}+\mathcal{L}^{local}_{l2v}$.


\subsection{Complexity Analysis.}
% \input{figs/pretrain-time}
% To democratize VLP, we deploy several strategies: \textit{i) data reduction}, we use a subset of pre-training dataset to train our method; \textit{ii) region feature}, region features enable us to use only few regions to represent a video frame, while CNN and ViT need hundreds of feature vectors or patches; and \textit{iii) sparse frame sampling}, we only sample 1 frame per video to improve efficiency. 
% We give quantitative results to show the efficiency of our method and analyze the key factors.
Previous offline-feature-based VLP methods~\cite{li2020hero,zhu2020actbert,yang2021taco} are criticized for excessive demand on memory and computation.
However, we claim that our method is more efficient that recent end-to-end methods~\cite{Bain_2021_ICCV,lei2021less,fu2021violet} overall.
Although we need to pay extra time to extract region features, it is negligible compared with the pre-training time that our method saves, especially we only need to extract them once but can reuse them for plenty of times.
When it comes to downstream tasks, the detector only needs to extract features for queries, as we can assume gallery features are pre-extracted and stored in practical.
Such extra time is also acceptable considering the performance improvements.
We give a detailed complexity analysis as follow.
\input{figs/pretrain-time}

\noindent\textbf{Pre-training.} We compare the pre-training time and R@1 on MSRVTT retrieval of our method with different settings and other methods.
Because different methods use different number of GPUs, we introduce GPU Hours, i.e., \textit{number of GPUs} $\times$ \textit{pre-training time}, to measure the computational cost.
As the results shown in Table~\ref{tab:pretrain-time}, our method is significantly more efficient than other methods. 
Our method achieves the best performance, even when we only use 20\% pre-training data and extremely sample only 1 frame per video.
Compared with the most efficient VLP method so far, i.e., ClipBERT~\cite{lei2021less}, our method save 85\% pre-training time.
% Even with so limited data, our method still surpasses the performance of other methods. 
The reason why the model pretrained with 50\% data performs better than those pretrained with more data is that finetuning results may not be strictly correlated with the data scale.
Zero-shot results reflect the impact of data scale more precisely.
As shown in Fig.~\ref{fig:data-scale} and \ref{fig:num-frame}, zero-shot results degrade slightly as the number of frames and the size of data decreases.
% In detail, when we reduce the number of sampling frames from 4 to 1, the pre-training time is reduce by 50\%. 
% The reduction of pre-training data also sharply decrease the pre-training time.
% By reduce 80\% pre-training data, the pre-training time is reduced by 87\%.
% In next section, we will show that even reducing 80\% data, our method still performs better than state-of-the-art methods.

Besides the whole pre-training, we also explore the running time of a training loop.
We compare our method with Frozen~\cite{Bain_2021_ICCV} and VIOLET~\cite{fu2021violet} to show the efficiency of our method.
% To make a fair comparison, the batchsize of all methods is set to 16, each video is sampled 1 frame and mixed precision is not used.
As the results shown in Fig.~\ref{fig:train-time}, our method requires much less time than Frozen~\cite{Bain_2021_ICCV} and VIOLET~\cite{fu2021violet}.
The forward time of our method is only 43.8\% of Frozen's and 9.7\% of VIOLET's.
The backward time of our method is only 34.5\% of Frozen's and 9.9\% of VIOLET's.
% This contributes to two factors: \textit{i)} we use the original ViT~\cite{dosovitskiy2020vit}, which avoids time-consuming temporal modules; \textit{ii)} region features can represent a video with few vectors compared with CNN feature maps or dense patches, which accelerates self-attention in Transformer sharply. 

\noindent\textbf{Downstream Retrieval.}
We test the inference time of each model components on text-to-video retrieval.
We build up two galleries: \textbf{i)} test split of LSMDC that contains 1000 samples; \textbf{ii)} 12000 samples collected from WebVid's train split.
In practical, samples in gallery are pre-extracted, thus we record the running time of detection, feature extraction of a query and ranking.

As shown in Table~\ref{tab:infer-time-all}, detection costs around 100ms for a video.
Feature extraction of texts and videos takes very little time.
As the gallery expands, ranking time becomes the major consumption.
Considering the gallery capacity is usually larger than 12000 in practical, the extra time for detection is acceptable.
\input{tables/infer-time-all}

==> sections/4-Exp.tex <==
\section{Experiments}
% In this section, we first introduce pre-training datasets and downstream tasks in Section~\ref{pt data} and \ref{ds task}. Implementation details are described in Section~\ref{imple}. 
% In Section~\ref{rwa}, we verify the effectiveness of the proposed region-word alignment. 
% % The pre-training efficiency is analyzed in Section~\ref{pt efficiency}. 
% Comparisons with state-of-the-art methods are demonstrated in Section~\ref{com}.
% Finally, we conduct ablation study and visualization in Section~\ref{ablation} and Section~\ref{visua} respectively.

\subsection{Pre-training Datasets}
\label{pt data}
Following the recent works~\cite{Bain_2021_ICCV,fu2021violet}, we involve a video-language dataset and an image-language dataset to pre-train our model.
\textbf{i) WebVid2.5M (WebVid)} consists of 2.5M video-language pairs collected from web.
WebVid contains manually generated captions that are well-formed sentences and well-aligned with videos. 
% Compared with larger but noisy datasets, HowTo100M~\cite{miech2019howto100m}, WebVid enables learning joint video-language representations with less data and pre-training time. 
\textbf{ii) Google Conceptual Captions (CC3M)} consists of 3.3M image-language pairs. 
Images and raw textual descriptions are harvested from the web following a similar process to WebVid.

\subsection{Downstream Tasks}
\label{ds task}
We evaluate our method on text-to-video retrieval and video question answering, across 7 downstream tasks. For \textbf{Text-to-Video Retrieval}, we report results on
\textit{i)} \textbf{MSRVTT};
\textit{ii)} \textbf{DiDeMo};
\textit{iii)} \textbf{LSMDC} and
\textit{iv)} \textbf{MSVD}. 
We adopt the common R@K (K=1, 5, 10) metric and Median Rank (MedR) to measure the performance of retrieval.

For \textbf{Video Question Answering}, we evaluate the performance on multiple-choice and open-ended settings:
\textit{i)} \textbf{MSRVTT Multiple Choice};
\textit{ii)} \textbf{MSRVTT-QA} and 
\textit{iii)} \textbf{MSVD-QA}.
The metric of video question answering tasks is accuracy. More details are provided in Supplementary.

% \noindent\textbf{Text-to-Video Retrieval.}
% \textit{i)} \textbf{MSRVTT} consists of 10K videos with 200K captions. We follow the previous works~\cite{Bain_2021_ICCV,liu2019use} to train on 9K train and validation videos and test on the 1K test set.
% \textit{ii)} \textbf{DiDeMo} consists of 10K videos with 40K captions. We concatenate all sentences of a video to a single query as previous works~\cite{Bain_2021_ICCV,lei2021less}, and we do not use the ground-truth localization annotations of this dataset.
% \textit{iii)} \textbf{LSMDC} contains 128K videos. We follow the setting in \cite{Bain_2021_ICCV} to test our method on the 1K test set.
% \textit{iv)} \textbf{MSVD} contains 1,970 videos. We split MSVD into 1,200, 100 and 670 videos as the train, validation and test set. 

% We adopt the common R@K (K=1, 5, 10) metric and Median Rank (MedR) to measure the performance of retrieval.


% \noindent\textbf{Video Question Answering.}
% \textit{i)} \textbf{MSRVTT Multiple Choice} is a question answering task that videos are questions and captions are answer candidates. Each video has 5 captions, and only caption is the positive one.
% \textit{ii)} \textbf{MSRVTT-QA} is based on MSRVTT dataset. 243K open-ended questions and 1500 answers are annotated.
% \textit{iii)} \textbf{MSVD-QA} is based on MSVD dataset. It contains a total number of 1,970 videos and 50,505 question-answer pairs.
% The metric of video question answering tasks is accuracy.

\subsection{Implementation Details}
\label{imple}
% \noindent\textbf{Input.}
% We adopt Faster RCNN~\cite{anderson2018bottom} to extract 2048-dimensional region features from videos.
% It was trained on Visual Genome~\cite{krishna2017visual} for object detection and attribute classification.
% To encode the location information for each region, we follow UNITER~\cite{chen2020uniter} to project a 7-dimensional vector (normalized four coordinates, width, height, and area) to a 2048-dimensional location vector.
% The final region feature is obtained by summing up the extracted region feature and location vector.
% For textual inputs, we follow BERT~\cite{devlin2018bert} and tokenize the sentence into WordPieces~\cite{wu2016google}.

% \noindent\textbf{Model.}
% For the video encoder, we utilize the original ViT~\cite{dosovitskiy2020vit} to refine region features.
% For the language encoder, to improve efficiency, we adopt DistillBERT~\cite{sanh2019distilbert} as LE, which has 40\% less parameters than BERT~\cite{devlin2018bert} and preserves over 95\% of BERT's performance.

% \noindent\textbf{Training.}
We implement our method with Pytorch and train all models on Tesla V100 GPUs with a batch size of 128 per GPU. We use the Adam optimizer with different learning rate schedule on pre-training and downstream finetuning.    
For pre-training, we train our model in 50 epochs using an initial learning rate of $1\times10^{-5}$. 
The learning rate decays to 1/10 of the previous one at 30 and 40 epochs.  
For fine-tuning, all experiments on downstream tasks are trained in 10 epochs.
We densely sample 8 frames for each video. 
The initial learning rate is $1\times10^{-5}$ and decays to 1/10 at 2, 4 and 8 epochs.
% In detail, for text-to-video retrieval, we sum up the global and local similarity as the final similarity between video and text. 
% The final similarity is used to rank all video-language pairs.
% For MSRVTT Multiple Choice, we directly use the model finetuned for MSRVTT retrieval to evaluate the performance.
% For MSRVTT-QA and MSVD-QA that are open-ended question answering tasks, we adopt the framework in BUTD~\cite{anderson2018bottom}, which uses a multi-label classifier based on region features and text features of questions to perform question answering task.

\subsection{Analysis of Region-Word Alignment}
\label{rwa}
\noindent\textbf{Effectiveness.}
% \input{tables/rwa-effect}
% \input{tables/rwa-new}
To demonstrate the effectiveness of our proposed region-word alignment (RWA), we perform our method with and without RWA. 
For the model without RWA (i.e., Base), the pre-training objective is modified into $\mathcal{L}=\mathcal{L}^{\text{global}}_{\text{v2l}}+\mathcal{L}^{\text{global}}_{\text{l2v}}$.
Furthermore, we compare RWA to other fine-grained alignment methods, e.g., TACo~\cite{yang2021taco} and FILIP~\cite{yao2022filip}.

The results on MSRVTT retrieval are shown in Table~\ref{tab:rwa-effect}. 
Specifically, RWA improves Base by 13.5 on R@1.
Compared to TACo~\cite{yang2021taco} and FILIP~\cite{yao2022filip}, RWA brings 6.2 and  improvements on R@1, respectively.
TACo and FILIP only align each region with the most relevant word, however, a region can correspond to multiple words.
Such cases are covered by RWA, thus, RWA brings more gain than TACo and FILIP.
\input{tables/rwa-new}

\noindent\textbf{Generalization.}
% \input{tables/rwa-gene}
We observe that RWA can seamlessly adapt to end-to-end methods.
To prove it, we add RWA to an end-to-end VLP methods, i.e.,  Frozen~\cite{Bain_2021_ICCV}, which divides the video frame into 196 non-overlapping patches as the input.
% ; \textbf{ii) Frozen-Crop}. We replace non-overlapping patches with crops of object regions from raw pixels.
The results on MSRVTT retrieval are shown in Table~\ref{tab:rwa-gene}.
RWA improves R@1 of Frozen by 4.1 and 3.0 for finetuning and zero-shot settings, respectively.
The gain demonstrates that RWA can generalize to other end-to-end VLP methods.
% The improvement on region-based method, i.e., Frozen-Crop, is more obvious.
% We argue that non-overlapping patches still contains noisy data, e.g., background, which easily causes misalignment between patches and words.
% The misalignment limits the improvement of RWA.

% To demonstrate the effectiveness of the proposed region-word alignment (RWA), we perform our method with and without RWA. 
% For the model without RWA, the pre-training objective is modified into $\mathcal{L}=\mathcal{L}^{global}_{v2l}+\mathcal{L}^{global}_{l2v}$.
% Further, to show the generalization of RWA, we integrate it into Frozen~\cite{Bain_2021_ICCV}. 

% The results on MSRVTT retrieval are shown Table~\ref{tab:rwa-gene}.
% In general, RWA brings a large margin for our method and Frozen for both finetuning and zero-shot settings.
% Specifically, RWA improves our method by 7.9 and 13.5 on R@1 for zero-shot and finetuning, respectively.
% It also improves the R@1 of Frozen by 2.6 and 1.4 for finetuning and zero-shot, respectively.
% The results verify that the proposed region-word alignment can effectively match video-language pairs.
% Meanwhile, the gains on Frozen demonstrate that such fine-grained alignment can generalize to other video-language pre-training methods.
% \input{tables/rwa}
% \input{figs/rwa+sampling}

% \subsection{Analysis of Pre-training Efficiency}
% \label{pt efficiency}
% To democratize VLP, we deploy several strategies: \textit{i) data reduction}, we use a subset of pre-training dataset to train our method; \textit{ii) region feature}, region features enable us to use only few regions to represent a video frame, while CNN and ViT need hundreds of feature vectors or patches; and \textit{iii) sparse frame sampling}, we only sample 1 frame per video to improve efficiency. We give quantitative results to show the efficiency of our method and analyze the key factors. 

% \noindent\textbf{Pre-training Time.}
% \input{figs/pretrain-time}
% We compare the pre-training time of our method with different settings and other methods.
% Because different methods use different number of GPUs, we introduce GPU Hours, i.e., \textit{number of GPUs} $\times$ \textit{pre-training time}, to measure the computational cost.
% As the results shown in Table~\ref{tab:pretrain-time}, our method is significantly more efficient than other methods, especially when we only use 20\% pre-training data and sample 1 frame per video.
% In detail, when we reduce the number of sampling frames from 4 to 1, the pre-training time is reduce by 50\%. 
% The reduction of pre-training data also sharply decrease the pre-training time.
% By reduce 80\% pre-training data, the pre-training time is reduced by 87\%.
% In next section, we will show that even reducing 80\% data, our method still performs better than state-of-the-art methods.

% Besides the whole pre-training, we also explore the running time of a training loop.
% We compare our method with Frozen~\cite{Bain_2021_ICCV} and VIOLET~\cite{fu2021violet} to show the efficiency of our method.
% To make a fair comparison, the batchsize of all methods is set to 16, each video is sampled 1 frame and mixed precision is not used.
% As the results shown in Fig.~\ref{fig:train-time}, our method requires much less time than Frozen~\cite{Bain_2021_ICCV} and VIOLET~\cite{fu2021violet}.
% The forward time of our method is only 43.8\% of Frozen's and 9.7\% of VIOLET's.
% The backward time of our method is only 34.5\% of Frozen's and 9.9\% of VIOLET's.
% This contributes to two factors: \textit{i)} we use the original ViT~\cite{dosovitskiy2020vit}, which avoids time-consuming temporal modules; \textit{ii)} region features can represent a video with few vectors compared with CNN feature maps or dense patches, which accelerates self-attention in Transformer sharply. 

% To specify how the sparse region sampling affects the efficiency, we give the running time of a training loop in Table~\ref{fig:train-time}. 

% \noindent\textbf{Impact of Sampling Strategy.}
% Although sparse sampling strategy reduce the pre-training time, we need to make sure the performance of pre-training is still good.
% To quantitatively evaluate the impact of sparsely sampling strategy, we compare four models that sample 1, 2, 4, 8 frames per video respectively. 

% The results on MSRVTT retrieval are shown in Fig.~\ref{fig:frame-number}. 
% In general, the number of frames does not show obvious impact on downstream tasks.
% As the number of frames increases, the zero-shot results are improved, whereas the finetuning results are very close. Even when the number of frames is set to 8, the finetuning result is the worst.

% \noindent\textbf{Impact of Dataset Scale.}
% % \input{figs/data-scale}
% To reach an extremely efficient video-language pre-training, we drastically reduce the pre-training data scale.
% In general, the reduction of pre-training data causes heavy performance drop of VLP models.
% However, benefitting from region features that focus on meaningful and salient regions, even with 20\% pre-training data, our method can still obtain results closing to the one with 100\% data.
% To verify it, we compare our methods that are pre-trained with different scales of data, i.e., 20\%, 50\%, 60\%, 80\% and 100\%, on MSRVTT retrieval.
% Further, to figure out whether region features or region-word alignment makes our method can be trained very limited data, we give the results of our method on different data scales without region-word alignment.

% As the results shown in Figure~\ref{fig:local-data-scale}, as the data scale decreases to 50\%, R@1 of different scales are very close for both finetuning and zero-shot settings.
% Only if the scale drops to 20\%, R@1 for zero-shot and finetuning decreases to 21.8 and 34.6 respectively, which is obviously worse than other scales.
% However, such performance is still better than other state-of-the-art methods, e.g., Frozen~\cite{Bain_2021_ICCV}, SupportSet~\cite{patrick2021supportset} and TACo~\cite{yang2021taco}.
% The results in Fig.~\ref{fig:global-data-scale} demonstrate that region features are the main reason why our method can be trained with very limited data.
% Although the performance of our method drops heavily without region-word alignment, the results with different scales are very close.

\subsection{Comparisons with State-of-the-art}
\label{com}
We compare our method with state-of-the-art methods on text-to-video retrieval and video question answering tasks. All results in this section is based on the model that samples 1 frame per video during pre-training.

\noindent\textbf{Text-to-Video Retrieval.}
\input{tables/retrieval}
Table~\ref{tab:video_retrieval} summarizes the results on text-to-video retrieval.
Across all four tasks, our method achieves significant improvement compared with previous methods in both finetuning and zero-shot settings. 
On LSMDC, our method outperforms the AVLNet~\cite{rouditchenko2021cascaded} by 8.2 on R@1. Similarly, on MSRVTT, our method surpasses Frozen~\cite{Bain_2021_ICCV} by 5.0 and 5.3 on R@1 for finetuning and zero-shot settings.
For DiDeMo and MSVD, our method brings more than 10 improvement compared with existing best methods.
Another advantage of our method is that our zero-shot performance significantly surpasses other methods.
This means that our method builds up a good alignment between video and language during pre-training and generalizes well on different datasets.

\noindent\textbf{Video Question Answering.}
\input{tables/video_qa}
Table~\ref{tab:video_qa} summarizes the results on video question answering tasks. 
On MSRVTT MC, our method obtains accuracy of 92.4\%, which outperforms prior state-of-the-art VideoCLIP~\cite{xu2021videoclip} by 0.5\%.
On MSRVTT-QA and MSVD-QA, our method achieves accuracy of 38.3\% and 39.5\%.
Compared to ClipBERT~\cite{lei2021less}, our method brings 0.9\% improvement on MSRVTT-QA.
It also surpasses DualVGR~\cite{wang2021dualvgr} by 0.5\% on MSVD-QA. 
% Our method only performs worse than VIOLET~\cite{fu2021violet} and JustAsk~\cite{Yang_2021_ICCV}. 
% The main reason that the pre-training data we used is much less that VIOLET and JustAsk, where VIOLET and JustAsk are pre-trained with 185.8M and 69M video-text pairs.

% \input{tables/retrieval}
% \input{tables/msrvtt_retrieval}
% \input{tables/didemo_retrieval}
% \input{tables/lsmdc_retrieval}
% \input{tables/msvd_retrieval}
% \input{tables/msrvtt_mc}
% \input{tables/qa}
% \input{tables/video_qa}

% \subsection{Ablation Study}
% \label{ablation}

% \noindent\textbf{Effectiveness of Loss.}

% \noindent\textbf{Impact of Sampling Strategy.}

% \noindent\textbf{Impact of Dataset Scale.}

% \noindent\textbf{Pre-training Time.}
% \input{tables/dataset}
% \input{tables/trick}
% \input{tables/crop}
% \input{tables/infer-time}

\subsection{Ablation Study}
\label{ablation}

\noindent\textbf{Data Scale.}
% \input{tables/dataset}
% \input{figs/data-scale-gene}
In this section, we explore the impact of different pre-training data scales.
We compare models that are pre-trained with different scales of data, i.e., 20\%, 50\%, 60\%, 80\% and 100\%, on MSRVTT retrieval.
As shown in Fig.~\ref{fig:data-scale}, as the data scale decreases to 50\%, R@1 of different scales are very close.
Only if the scale drops to 20\%, R@1 decreases to 34.6, which is still better than other state-of-the-art methods' results, e.g., Frozen~\cite{Bain_2021_ICCV}, SupportSet~\cite{patrick2021supportset} and TACo~\cite{yang2021taco}.
The model without RWA has a similar trend to the one with RWA across different scales.
It demonstrates that region features are the main reason why our method can be trained with very limited data.
\input{figs/data-scale-gene}

Furthermore, to verify whether our method can generalize to larger datasets or not, we evaluate our method pre-trained with more data on MSRVTT retrieval.
Specifically, we add a subset of Conceptual 12M~\cite{changpinyo2021cc12m} as pre-training data.
The subset contains 7M samples that are disjoint from CC3M, denoted as CC7M.
As results shown in Table~\ref{tab:data-gene}, CC7M can further improve the results of our method.
It verifies that our method can extend to massive data to achieve better performance.
An interesting observation is that adding data from original datasets (i.e., WebVid and CC3M) cannot improve the performance, while adding extra  data from a different domain (i.e., CC7M) can.
This observation inspires us that the diversity of data plays an important role in VLP.

% To reach an extremely efficient video-language pre-training, we drastically reduce the pre-training data scale.
% In general, the reduction of pre-training data causes heavy performance drop of VLP models.
% However, benefitting from region features that focus on meaningful and salient regions, even with 20\% pre-training data, our method can still obtain results closing to the one with 100\% data.
% To verify it, we compare our methods that are pre-trained with different scales of data, i.e., 20\%, 50\%, 60\%, 80\% and 100\%, on MSRVTT retrieval.
% Further, to figure out whether region features or region-word alignment makes our method can be trained very limited data, we give the results of our method on different data scales without region-word alignment.

% As the results shown in Figure~\ref{fig:data-scale}, as the data scale decreases to 50\%, R@1 of different scales are very close for both finetuning and zero-shot settings.
% Only if the scale drops to 20\%, R@1 for zero-shot and finetuning decreases to 21.8 and 34.6 respectively, which is obviously worse than other scales.
% However, such performance is still better than other state-of-the-art methods, e.g., Frozen~\cite{Bain_2021_ICCV}, SupportSet~\cite{patrick2021supportset} and TACo~\cite{yang2021taco}.
% The results in Fig.~\ref{fig:data-scale} demonstrate that region features are the main reason why our method can be trained with very limited data.
% Although the performance of our method drops heavily without region-word alignment, the results with different scales are very close.

\noindent\textbf{Number of Regions.}
To determine how many regions can represent a video frame, we vary the number of regions and test our method's performance on MSRVTT retrieval.
As the results shown in Fig.~\ref{fig:num-obj}, R@1 is improved as the number of regions increases from 10 to 30.
When the number continues to increase, the gain on R@1 is not obvious.
The results verify our claim that \textit{a frame is actually worth around 30 objects}.

\noindent\textbf{Sampling Strategy.}
% \input{figs/num-frame-obj}
% Although sparse sampling strategy reduce the pre-training time, we need to make sure the performance of pre-training is still good.
To quantitatively evaluate the impact of sparsely sampling strategy, we compare four models that sample 1, 2, 4, 8 frames per video during pre-training respectively.
When conducting downstream tasks, 8 frames are sampled.
\input{figs/num-frame-obj}

The results on MSRVTT retrieval are shown in Fig.~\ref{fig:num-frame}. 
In general, the number of frames does not show obvious impact on downstream tasks.
% As the number of frames increases, the zero-shot results are improved, whereas the finetuning results are very close. 
% Even when the number of frames is set to 8, the finetuning result is the worst.
As the number of frames varies, the performance for zero-shot and finetuning settings is close.
This means that we can sparsely sampling frames during pre-training to save pre-training time.
\input{tables/comp}

\noindent\textbf{Word of Interest.}
% \input{tables/trick}
% \input{tables/comp}
% \input{figs/comp-infer}
% Both TACo~\cite{yang2021taco} and our method tries to select the  
We refine attention weights in Eq (\ref{eq:ref_attn}) to choose the most relevant words with respect to a video.
% In this section, we verify the effect of different model explorations.
To determine the effect of this operation, we compare it with another operation, i.e., \textbf{Select Token}, which manually selects nouns and verbs as the input caption.
Because nouns and verbs usually contain more semantics than other types of words~\cite{yang2021taco}.
Results on MSRVTT retrieval are shown in Table~\ref{tab:ablation}, our method performs the best, and \textbf{Select Token} even performs worse than baseline.
This prove that a proper strategy to find the most relevant words is necessary, while naive manual selection is ineffective.
% both our method and \textbf{Select Token} perform better than baseline.
% Our method achieves close results to \textbf{Select Token}.
% This prove that our method indeed finds the most relevant words.

\noindent\textbf{Region Selection.}
To compare different region selection methods: \textbf{i) Sorted Selection} and \textbf{ii) Track Object}, we give their performance on MSRVTT retrieval.
As shown in Table~\ref{tab:ablation}, \textbf{Sorted Selection} performs better than \textbf{Track Object}.
This means that discriminative region features are more important for VLP than covering more object categories.

% \noindent\textbf{Inference Efficiency.}
% \input{tables/infer-time}
\noindent\textbf{Temporal Modelling.}
Frozen utilizes TimeSformer~\cite{bertasius2021space} as the backbone, which proposes a time-attention layer to model temporal information.
In our work, we rely on temporal position embeddings to model temporal information.
To evaluate the impact of time-attention layer, we conduct experiments on MSRVTT retrieval.
As shown in Table~\ref{tab:ablation}, time-attention layer cannot bring improvement to our method.
Thus, in our framework, temporal position embeddings are enough to model temporal clues.
\subsection{Visualization}
\label{visua}
% \input{figs/vis}
We also provide qualitative results on Fig.~\ref{fig:vis} to show the alignment between video and language.
% \input{figs/vis}
In Fig.~\ref{fig:region-word-vis}, we visualize the attended regions with respect to the most relevant word in the sentence.
We observe that not only nouns are connected with corresponding regions, even verbs, such as ``see" and ``smile", are also aligned with relevant regions.
Fig.~\ref{fig:video-caption-vis} shows the attention heatmap between video frames and corresponding sentence.
Regions that are relevant to the sentence description show higher attention weights than others.
Visualization verifies that our proposed global-local alignment successfully connects video and language from coarse-grained to fine-grained level.
\input{figs/vis}

==> sections/5-Con.tex <==
\section{Conclusion}
In this work, we introduce the most efficient video-language pre-training method to date, which revitalizes region features with a bidirectional region-word alignment regularization.
% Region features that focus on limited salient areas enables our method to be extremely time-saving, because the model can be trained with a small number of data. 
Region features that focus on salient areas remove spatial visual redundancy, which enables our VLP method to be extremely time-saving.
The region-word alignment constraint builds up a fine-grained connection between video and language.
% It can even generalize to end-to-end VLP models.
Experimental results on downstream tasks and visualization prove the efficiency and effectiveness of our method.

==> tables/clip.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{lllll}
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{4}{c}{\textbf{Text$\rightarrow$Video}}                       \\
\multicolumn{1}{l|}{}                                 & \textbf{R@1}  & \textbf{R@5}  & \textbf{R@10} & \textbf{MedR} \\ \hline
\multicolumn{1}{l|}{SFCLIP~\cite{portillo2021straightforward}}                               & 40.3          & 69.7          & 79.2          & 2.0           \\
\multicolumn{1}{l|}{CLIP2Video~\cite{fang2021clip2video}}                       & 45.6          &     72.4      &     80.7     & 2.0           \\
\multicolumn{1}{l|}{CLIP4CLIP~\cite{luo2021clip4clip}}                           & 43.1          & 70.4          & 80.8          & 2.0           \\
\multicolumn{1}{l|}{Ours}                    & 40.5 & 69.1 & 79.4 & 2.0  \\ \hline
\multicolumn{1}{l|}{Ours (WebVid+CC3M)}                    & 36.0 & 61.0 & 71.8 & 3.0  \\ \hline
\multicolumn{5}{l}{Zero-shot}                                                                                         \\ \hline
\multicolumn{1}{l|}{CLIP4CLIP~\cite{luo2021clip4clip}}                    & 30.6 & 54.4 & 64.3 & 4.0    \\
\multicolumn{1}{l|}{Ours}                    & 26.8 & 51.0 & 61.7 & 5.0    \\ \hline
\multicolumn{1}{l|}{Ours (WebVid+CC3M)}                    & 24.0 & 44.0 & 52.6 & 8.0    \\ \hline
\end{tabular}%
}
\vspace{2mm}
\caption{Comparisons with State-of-the-art methods based on CLIP's weights on MSRVTT Retrieval. Ours (WebVid+CC3M) denotes our method pre-trained with WebVid and CC3M.}
\label{tab:clip}
\end{table}

==> tables/comp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
\vspace{-4mm}
\begin{tabular}{c|c|c|c|llll}
\hline
                                     &                                      &                                &                                  & \multicolumn{4}{c}{Text$\rightarrow$Video} \\
\multirow{-2}{*}{Refine Attention}   & \multirow{-2}{*}{Select Token}       & \multirow{-2}{*}{Track Object} & \multirow{-2}{*}{Temporal Model} & R@1    & R@5   & R@10  & MedR  \\ \hline
-                                    & -                                    & -                              & -                                &    34.5    &  58.3     &  70.2     &   3.0    \\
\rowcolor{LightCyan} 
$\checkmark$                         & -                                    & -                              & -                                & \textbf{36.0}   & \textbf{61.0}  & \textbf{71.8}  & \textbf{3.0}   \\
-            & $\checkmark$ & -                              & -                                &    32.8    &  55.5     &  69.2     &  3.0     \\
$\checkmark$ & -                                    & $\checkmark$                   & -                                & 33.6   & 59.2  & 69.7  & 3.0   \\
$\checkmark$ & -                                    & -                              & $\checkmark$                     & 35.9   & 60.8  & 71.8  & 3.0   \\ \hline
\end{tabular}
\vspace{2mm}
\caption{Ablation study of different model explorations. The first row denotes a baseline and the colored row denotes our method.}
\label{tab:ablation}
\vspace{-8mm}
\end{table}

==> tables/crop.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{llll}
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{Method}} & \multicolumn{3}{c}{Text Video} \\
\multicolumn{1}{l|}{}                        & R@1      & R@5      & R@10     \\ \hline
\multicolumn{1}{l|}{Frozen-Crop}             & 18.3     & 36.0     & 47.3     \\ \hline
\multicolumn{1}{l|}{Frozen-Crop+RWA}         & 32.1     & 56.3     & 66.9     \\ \hline
\multicolumn{4}{l}{Zero-shot}                                                 \\ \hline
\multicolumn{1}{l|}{Frozen-Crop}             & 13.2     & 29.2     & 38.2     \\ \hline
\multicolumn{1}{l|}{Frozen-Crop+RWA}         & 21.5     & 39.5     & 49.1     \\ \hline
\end{tabular}
\end{table}

==> tables/dataset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{l|lll}
\hline
\multirow{2}{*}{Data} & \multicolumn{3}{c}{Text Video} \\
                      & R@1      & R@5      & R@10     \\ \hline
WebVid+CC3M           & 36.0     & 61.0     & 71.8     \\
CC3M+CC7M             & 38.7     & 63.8     & 73.9     \\
WebVid+CC3M+CC7M      & 39.6     & 64.8     & 73.8     \\ \hline
\end{tabular}
\end{table}

==> tables/didemo_retrieval.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lllll}
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{4}{c}{\textbf{Text Video}}                       \\
\multicolumn{1}{l|}{}                                 & \textbf{R@1}  & \textbf{R@5}  & \textbf{R@10} & \textbf{MedR} \\ \hline
\multicolumn{1}{l|}{S2VT}                             & 11.9          & 33.6          & -             & 13.0          \\
\multicolumn{1}{l|}{FSE}                              & 13.9          & 36.0          & -             & 11.0          \\
\multicolumn{1}{l|}{ClipBERT}                         & 20.4          & 44.5          & 56.7          & 7.0           \\
\multicolumn{1}{l|}{Frozen}                           & 31.0          & 59.8          & 72.4          & 3.0           \\ \hline
\multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{41.4} & \textbf{67.6} & \textbf{77.6} & \textbf{2.0}  \\ \hline
\multicolumn{5}{l}{Zero-shot}                                                                                         \\ \hline
\multicolumn{1}{l|}{Frozen}                           & 21.1          & 46.0          & 56.2          & 7.0           \\
\multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{29.6} & \textbf{53.0} & \textbf{65.1} & \textbf{4.0}  \\ \hline
\end{tabular}%
}
\end{table}

==> tables/infer-time-all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\vspace{-8mm}
\begin{tabular}{l|cc|cc}
\hline
\multirow{2}{*}{Components} & \multicolumn{2}{c|}{12000 Samples}                                   & \multicolumn{2}{c}{1000 Samples}                                     \\ \cline{2-5} 
                            & \multicolumn{1}{c|}{Text$\rightarrow$Video} & Video$\rightarrow$Text & \multicolumn{1}{c|}{Text$\rightarrow$Video} & Video$\rightarrow$Text \\ \hline
Language Encoder            & \multicolumn{1}{c|}{5.6ms}                  & -                      & \multicolumn{1}{c|}{4.8ms}                  & -                      \\
Video Encoder               & \multicolumn{1}{c|}{-}                      & 17.6ms                 & \multicolumn{1}{c|}{-}                      & 16.4ms                 \\
Detector                    & \multicolumn{1}{c|}{-}                      & 103.2ms                & \multicolumn{1}{c|}{-}                      & 103.2ms                \\ \hline
Rank                        & \multicolumn{1}{c|}{372.2ms}                & 345.8ms                & \multicolumn{1}{c|}{31.8ms}                 & 30.0ms                 \\ \hline
\end{tabular}
\vspace{3mm}
\caption{Inference time of each model component. Because the length of sentence and size of video frames are different in WebVid and LSMDC, inference time on language and video encoders is different.}
\vspace{-14mm}
\label{tab:infer-time-all}
\end{table}

==> tables/infer-time.tex <==
\begin{table}[]
\begin{tabular}{l|c|c|c|c}
\hline
Task       & Text & Video & Detect  & Rank    \\ \hline
Text Video & 5.6ms    & -         & -       & 372.2ms \\ \hline
Video Text & -        & 17.6ms    & 103.2ms & 345.8ms \\ \hline
\end{tabular}
\end{table}

==> tables/lsmdc_retrieval.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lllll}
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{4}{c}{\textbf{Text Video}}                       \\
\multicolumn{1}{l|}{}                                 & \textbf{R@1}  & \textbf{R@5}  & \textbf{R@10} & \textbf{MedR} \\ \hline
\multicolumn{1}{l|}{JSFusion}                         & 9.1           & 21.2          & 34.1          & 36.0          \\
\multicolumn{1}{l|}{MEE}                              & 9.3           & 25.1          & 33.4          & 27.0          \\
\multicolumn{1}{l|}{CE}                               & 11.2          & 26.9          & 34.8          & 25.3          \\
\multicolumn{1}{l|}{MMT}                              & 12.9          & 29.2          & 38.8          & 19.3          \\
\multicolumn{1}{l|}{AVLNet}                           & 17.0          & 38.0          & 48.6          & 11.0          \\
\multicolumn{1}{l|}{Dig}                              & 15.8          & 34.1          & 43.6          & 14.3          \\
\multicolumn{1}{l|}{Frozen}                           & 15.0          & 34.1          & 39.8          & 20.0          \\ \hline
\multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{25.2} & \textbf{45.5} & \textbf{54.5} & \textbf{7.0}  \\ \hline
\multicolumn{5}{l}{Zero-shot}                                                                                         \\ \hline
\multicolumn{1}{l|}{Ours}                             & 14.3          & 25.8          & 32            & 49.5          \\ \hline
\end{tabular}%
}
\end{table}

==> tables/mscoco.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{l|ccc|ccc}
\hline
\multirow{3}{*}{Method} & \multicolumn{3}{c|}{Text$\rightarrow$Image} & \multicolumn{3}{c}{Text$\rightarrow$Image} \\
                        & \multicolumn{3}{c|}{MSCOCO(1K)}             & \multicolumn{3}{c}{MSCOCO(5K)}             \\ \cline{2-7} 
                        & R@1           & R@5          & R@10         & R@1          & R@5          & R@10         \\ \hline
CAMP~\cite{wu2016value}                    & 58.5          & 87.9         & 95.0         & -            & -            & -            \\
SCAN~\cite{lee2018stacked}                    & 58.8          & 88.4         & 94.8         & -            & -            & -            \\ \hline
ViLBERT~\cite{lu2019vilbert}                 & -             & -            & -            & 38.6         & 69.3         & 80.4         \\
UNITER~\cite{chen2020uniter}                  & -             & -            & -            & 50.3         & 78.5         & 87.2         \\
Unicoder~\cite{huang-etal-2019-unicoder}                   & 69.7          & 93.5         & 96.2         & 48.4         & 76.7         & 85.9         \\
OSCAR~\cite{li2020oscar}                   & 75.7          & 95.2         & 98.3         & 54.0         & 80.8         & 88.5         \\
VinVL~\cite{zhang2021vinvl}                   & 78.8          & 96.1         & 98.5         & 58.1         & 83.2         & 90.1         \\
ViLT~\cite{kim2021vilt}                    & -             & -            & -            & 42.7         & 72.9         & 83.1         \\ \hline
Ours                    & 60.3          & 89.4         & 95.4         & 37.9         & 68.4         & 79.6         \\ \hline
\end{tabular}%
}
\vspace{2mm}
\caption{Comparisons with State-of-the-art results on MSCOCO Text-to-Image Retrieval.}
\label{tab:mscoco}
\end{table}

==> tables/msrvtt_mc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{l|c}
\hline
\textbf{Method} & \multicolumn{1}{l}{\textbf{MSRVTT}} \\ \hline
JSFusion        & 83.4                                \\
ActBERT         & 85.7                                \\
ClipBERT        & 88.2                                \\
VideoCLIP       & 92.1                                \\
MERLOT          & 90.9                                \\
VIOLET          & 91.9                                \\ \hline
\textbf{Ours}   & \textbf{92.2}                       \\ \hline
\end{tabular}%
}
\end{table}

==> tables/msrvtt_retrieval.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcllll}
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{PT Datasets}}} & \multicolumn{4}{c}{\textbf{Text Video}}                       \\
\multicolumn{1}{l|}{}                                 & \multicolumn{1}{c|}{}                                      & \textbf{R@1}  & \textbf{R@5}  & \textbf{R@10} & \textbf{MedR} \\ \hline
\multicolumn{1}{l|}{JSFusion}                         & \multicolumn{1}{c|}{\multirow{3}{*}{-}}                    & 10.2          & 31.2          & 43.2          & 13.0          \\
\multicolumn{1}{l|}{CE}                               & \multicolumn{1}{c|}{}                                      & 20.9          & 48.8          & 62.4          & 6.0           \\
\multicolumn{1}{l|}{MMT}                              & \multicolumn{1}{c|}{}                                      & 26.6          & 57.1          & 69.6          & 4.0           \\ \hline
\multicolumn{1}{l|}{HERO}                             & \multicolumn{1}{c|}{\multirow{8}{*}{HowTo100M}}            & 16.8          & 43.4          & 57.7          & -             \\
\multicolumn{1}{l|}{ActBERT}                          & \multicolumn{1}{c|}{}                                      & 16.3          & 42.8          & 56.9          & 10.0          \\
\multicolumn{1}{l|}{MIL-NCE}                          & \multicolumn{1}{c|}{}                                      & 14.9          & 40.2          & 52.8          & 9.0           \\
\multicolumn{1}{l|}{UniVL}                            & \multicolumn{1}{c|}{}                                      & 21.2          & 49.6          & 63.1          & 6.0           \\
\multicolumn{1}{l|}{SupportSet}                       & \multicolumn{1}{c|}{}                                      & 30.1          & 58.5          & 69.3          & 3.0           \\
\multicolumn{1}{l|}{AVLNet}                           & \multicolumn{1}{c|}{}                                      & 27.1          & 55.6          & 66.6          & 4.0           \\
\multicolumn{1}{l|}{Dig}                              & \multicolumn{1}{c|}{}                                      & 31.2          & 62.8          & 76.4          & 3.0           \\
\multicolumn{1}{l|}{VideoCLIP}                        & \multicolumn{1}{c|}{}                                      & 30.9          & 55.4          & 66.8          & -             \\
\multicolumn{1}{l|}{TACo}                             & \multicolumn{1}{c|}{}                                      & 28.4          & 57.8          & 71.2          & 4.0           \\ \hline
\multicolumn{1}{l|}{ClipBERT}                         & \multicolumn{1}{c|}{COCO, VG}                              & 22.0          & 46.8          & 59.9          & 6.0           \\
\multicolumn{1}{l|}{Frozen~\cite{Bain_2021_ICCV}}                           & \multicolumn{1}{c|}{CC, WebVid}                            & 32.5          & \textbf{61.5} & 70.5          & 3.0           \\
\multicolumn{1}{l|}{\textbf{Ours}}                    & \multicolumn{1}{c|}{CC, WebVid}                            & \textbf{36.0} & 61.0          & \textbf{71.8} & \textbf{3.0}  \\ \hline
\multicolumn{6}{l}{Zero-shot}                                                                                                                                                      \\ \hline
\multicolumn{1}{l|}{MIL-NCE}                          & \multicolumn{1}{c|}{\multirow{4}{*}{HowTo100M}}            & 7.5           & 21.2          & 29.6          & 38.0          \\
\multicolumn{1}{l|}{SupportSet}                       & \multicolumn{1}{c|}{}                                      & 12.7          & 27.5          & 36.2          & 24.0          \\
\multicolumn{1}{l|}{TACo}                             & \multicolumn{1}{c|}{}                                      & 9.8           & 25.0          & 33.4          & 29.0          \\
\multicolumn{1}{l|}{VideoCLIP}                        & \multicolumn{1}{c|}{}                                      & 10.4          & 22.2          & 30.0          & -             \\ \hline
\multicolumn{1}{l|}{Frozen}                           & \multicolumn{1}{c|}{CC, WebVid}                            & 18.7          & 39.5          & 51.6          & 10.0          \\
\multicolumn{1}{l|}{\textbf{Ours}}                    & \multicolumn{1}{c|}{CC, WebVid}                            & \textbf{24.0} & \textbf{44.0} & \textbf{52.6} & \textbf{8.0}  \\ \hline
\end{tabular}%
}
\end{table}

==> tables/msrvtt_retrieval_brief.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lllll}
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{4}{c}{\textbf{Text Video}}                       \\
\multicolumn{1}{l|}{}                                 & \textbf{R@1}  & \textbf{R@5}  & \textbf{R@10} & \textbf{MedR} \\ \hline
\multicolumn{1}{l|}{MMT}                              & 26.6          & 57.1          & 69.6          & 4.0           \\
\multicolumn{1}{l|}{ActBERT}                          & 16.3          & 42.8          & 56.9          & 10.0          \\
\multicolumn{1}{l|}{SupportSet}                       & 30.1          & 58.5          & 69.3          & 3.0           \\
\multicolumn{1}{l|}{AVLNet}                           & 27.1          & 55.6          & 66.6          & 4.0           \\
\multicolumn{1}{l|}{TACo}                             & 28.4          & 57.8          & 71.2          & 4.0           \\
\multicolumn{1}{l|}{ClipBERT}                         & 22.0          & 46.8          & 59.9          & 6.0           \\
\multicolumn{1}{l|}{Frozen}                           & 32.5          & \textbf{61.5} & 70.5          & 3.0           \\
\multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{36.0} & 61.0          & \textbf{71.8} & \textbf{3.0}  \\ \hline
\multicolumn{5}{l}{Zero-shot}                                                                                         \\ \hline
\multicolumn{1}{l|}{SupportSet}                       & 12.7          & 27.5          & 36.2          & 24.0          \\
\multicolumn{1}{l|}{Frozen}                           & 18.7          & 39.5          & 51.6          & 10.0          \\
\multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{24.0} & \textbf{44.0} & \textbf{52.6} & \textbf{8.0}  \\ \hline
\end{tabular}%
}
\end{table}

==> tables/msvd_retrieval.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lllll}
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{4}{c}{\textbf{Text Video}}                       \\
\multicolumn{1}{l|}{}                                 & \textbf{R@1}  & \textbf{R@5}  & \textbf{R@10} & \textbf{MedR} \\ \hline
\multicolumn{1}{l|}{VSE}                              & 12.3          & 30.1          & 42.3          & 14.0          \\
\multicolumn{1}{l|}{VSE++}                            & 15.4          & 39.6          & 53.0          & 9.0           \\
\multicolumn{1}{l|}{MCues}                            & 20.3          & 47.8          & 61.1          & 6.0           \\
\multicolumn{1}{l|}{CE}                               & 19.8          & 49.0          & 63.8          & 6.0           \\
\multicolumn{1}{l|}{SupportSet}                       & 28.4          & 60.0          & 72.9          & 4.0           \\
\multicolumn{1}{l|}{Frozen}                           & 33.7          & 64.7          & 76.3          & 3.0           \\
\multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{50.9} & \textbf{78.9} & \textbf{87.0} & \textbf{1.0}  \\ \hline
\multicolumn{5}{l}{Zero-shot}                                                                                         \\ \hline
\multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{41.6} & \textbf{69.8} & \textbf{80.5} & \textbf{2}    \\ \hline
\end{tabular}%
}
\end{table}

==> tables/pretrain-time.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c}
\hline
\textbf{Method} & \textbf{Data Scale} & \textbf{GPU Hours} \\ \hline
Frozen          & 5.8M                & 4800               \\
UniVL           & 132M                & 2496               \\
MERLOT          & 180M                & 32768              \\
VIOLET          & 185.8M              & 2240               \\
ClipBERT        & 5.6M                & 768                \\ \hline
Ours (4F/100\%) & 5.8M                & 1600               \\
Ours (1F/100\%) & 5.8M                & 800                \\
Ours (1F/50\%)  & 2.9M                & 416                \\
Ours (1F/20\%)  & 1.2M                & 104                \\ \hline
\end{tabular}%
}
\end{table}

==> tables/qa.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{l|c|c}
\hline
\textbf{Method} & \multicolumn{1}{l|}{\textbf{MSRVTT}} & \multicolumn{1}{l}{\textbf{MSVD}} \\ \hline
SSML            & 35.0                                & 35.1                              \\
HCRN            & 35.6                                & 36.1                              \\
DualVGR         & 35.5                                & 39.0                              \\
ClipBERT        & 37.4                                & -                                 \\
JustAsk         & 43.1                                & 46.3                              \\
VIOLET          & 43.9                                & 47.9                              \\ \hline
Ours            & 38.3                                & 39.5                              \\ \hline
\end{tabular}%
}
\end{table}

==> tables/rwa-effect.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{l|lll}
\hline
\multirow{2}{*}{Method} & \multicolumn{3}{c}{Text Video} \\
                        & R@1      & R@5      & R@10     \\ \hline
Base                    & 22.5     & 48.1     & 59.5     \\ \hline
Base+TACo               & -        & -        & -        \\
Base+FILIP              & -        & -        & -        \\ \hline
Ours(Base+RWA)          & 36.0     & 61.0     & 71.8     \\ \hline
\end{tabular}
\end{table}

==> tables/rwa-gene.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{l|lll}
\hline
\multirow{2}{*}{Method} & \multicolumn{3}{c}{Text Video} \\
                        & R@1      & R@5      & R@10     \\ \hline
Frozen-Crop             & 18.3     & 36.0     & 47.3     \\
Frozen-Crop+RWA         & 32.1     & 56.3     & 66.9     \\ \hline
Frozen                  & 31.0     & 59.5     & 70.5     \\
Frozen+RWA              & 35.1     & 60.7     & 70.9     \\ \hline
\end{tabular}
\end{table}

==> tables/rwa-new.tex <==
\begin{table}[h]
\vspace{-6mm}
    \begin{subtable}[h]{0.5\textwidth}
        \centering
        \begin{tabular}{l|lll}
\hline
\multirow{2}{*}{Method} & \multicolumn{3}{c}{Text$\rightarrow$Video} \\
                        & R@1      & R@5      & R@10     \\ \hline
Base                    & 22.5     & 48.1     & 59.5     \\ \hline
TACo~\cite{yang2021taco}               & 29.6     & 59.7     & \textbf{72.7}        \\
Base+TACo               & 29.8     & 60.1     & 70.7        \\ 
Base+FILIP              & 27.8        & 55.0        & 65.1       \\ \hline
Ours(Base+RWA)          & \textbf{36.0}     & \textbf{61.0}     & 71.8     \\ \hline
\end{tabular}
       \caption{Comparison with other visual-language alignment methods on MSRVTT retrieval.}
       \label{tab:rwa-effect}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.5\textwidth}
        \centering
        \begin{tabular}{llll}
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{Method}} & \multicolumn{3}{c}{Text$\rightarrow$Video} \\
\multicolumn{1}{l|}{}                        & R@1          & R@5          & R@10         \\ \hline
\multicolumn{1}{l|}{Frozen}                  & 31.0         & 59.5         & 70.5         \\ 
\multicolumn{1}{l|}{Frozen+RWA}              & 35.1         & 60.7         & 70.9         \\ \hline
\multicolumn{4}{l}{Zero-shot}                                                             \\ \hline
\multicolumn{1}{l|}{Frozen}                  & 18.7         & 39.5         & 51.6         \\ 
\multicolumn{1}{l|}{Frozen+RWA}              & 21.7         & 42.2         & 52.2         \\ \hline
\end{tabular}
        \caption{Results on MSRVTT retrieval when cooperating with Frozen.}
        \label{tab:rwa-gene}
     \end{subtable}
     \caption{Effectiveness and generalization ability of our region-word alignment.}
     \label{tab:rwa-new}
     \vspace{-10mm}
\end{table}

==> tables/rwa.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lllll}
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{4}{c}{\textbf{Text Video}}                       \\
\multicolumn{1}{l|}{}                                 & \textbf{R@1}  & \textbf{R@5}  & \textbf{R@10} & \textbf{MedR} \\ \hline
\multicolumn{1}{l|}{Frozen+RWA}                       & 35.1          & 60.7          & 70.9          & 3.0           \\
\multicolumn{1}{l|}{Frozen}                           & 32.5          & \textbf{61.5} & 70.5          & 3.0           \\ \hline
\multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{36.0} & 61.0          & \textbf{71.8} & \textbf{3.0}  \\
\multicolumn{1}{l|}{Ours w/o RWA}                     & 22.5          & 48.1          & 59.5          & 6.0           \\ \hline
Zero-shot                                             &               &               &               &               \\ \hline
\multicolumn{1}{l|}{Frozen+RWA}                       & 20.1          & 37.5          & 49.3          & 11.0          \\
\multicolumn{1}{l|}{Frozen}                           & 18.7          & 39.5          & 51.6          & 10.0          \\ \hline
\multicolumn{1}{l|}{\textbf{Ours}}                    & \textbf{24.0} & \textbf{44.0} & \textbf{52.6} & \textbf{8.0}  \\
\multicolumn{1}{l|}{Ours w/o RWA}                     & 16.1          & 34.9          & 44.2          & 16.0          \\ \hline
\end{tabular}%
}
\end{table}

==> tables/trick.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{c|c|lll}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Obj Track}} & \multicolumn{1}{c|}{\multirow{2}{*}{Temp Attn}} & \multicolumn{3}{c}{Text Video} \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                           & R@1      & R@5      & R@10     \\ \hline
-                                               & -                                               & 36.0     & 61.0     & 71.8     \\
$\checkmark$                                               & -                                               & 33.6     & 59.2     & 69.7     \\
-                                               & $\checkmark$                                               & 35.9     & 60.8     & 71.8     \\ \hline
\end{tabular}
\end{table}
